Two Warm Neptunes transiting HIP 9618 revealed by TESS & Cheops

HIP 9618 (HD 12572, TOI-1471, TIC 306263608) is a bright ($G=9.0$ mag) solar analogue. TESS photometry revealed the star to have two candidate planets with radii of $3.9 \pm 0.044$ $R_\oplus$ (HIP 9618 b) and $3.343 \pm 0.039$ $R_\oplus$ (HIP 9618 c). While the 20.77291 day period of HIP 9618 b was measured unambiguously, HIP 9618 c showed only two transits separated by a 680-day gap in the time series, leaving many possibilities for the period. To solve this issue, CHEOPS performed targeted photometry of period aliases to attempt to recover the true period of planet c, and successfully determined the true period to be 52.56349 d. High-resolution spectroscopy with HARPS-N, SOPHIE and CAFE revealed a mass of $10.0 \pm 3.1 M_\oplus$ for HIP 9618 b, which, according to our interior structure models, corresponds to a $6.8\pm1.4\%$ gas fraction. HIP 9618 c appears to have a lower mass than HIP 9618 b, with a 3-sigma upper limit of $< 18M_\oplus$. Follow-up and archival RV measurements also reveal a clear long-term trend which, when combined with imaging and astrometric information, reveal a low-mass companion ($0.08^{+0.12}_{-0.05} M_\odot$) orbiting at $26^{+19}_{-11}$ au. This detection makes HIP 9618 one of only five bright ($K<8$ mag) transiting multi-planet systems known to host a planet with $P>50$ d, opening the door for the atmospheric characterisation of warm ($T_{\rm eq}<750$ K) sub-Neptunes.

==> TOI1471_finalmodel_TOI1471_notessgp_norollangelgp_wpipe_nottvs_3rvpoly_noeccentricity_noldprior_20220824_trace_modeltable1.tex <==
Stellar temperature, \teff{}  [K]  & $\mathcal{N}(\mu=5640,\sigma=30) $ &  $ 5641.0 \pm 31.0 $  \\
Stellar radius, $R_s$ [$R_\oplus$] & $\mathcal{N}(\mu=0.962,\sigma=0.008) $ &  $ 0.9622 \pm 0.0081 $  \\
log stellar surface gravity, \logg{}  [cgs] & $\mathcal{N}(\mu=4.47,\sigma=0.1) $ &  $ 4.45^{+0.015}_{-0.026} $  \\
Log RV semi-amplitude, $\log{K}$ & $\mathcal{N}(\mu=0.693147,\sigma=10)$ &  $ 1.08 \pm 0.17 $  \\
Log RV semi-amplitude, $\log{K}$ & $\mathcal{N}(\mu=0.693147,\sigma=10)$ &  $ 0.22^{+0.3}_{-0.49} $  \\
Quadratic LD, $u_{{\rm TESS},0} $  & $\mathcal{N}_{\mathcal{U}}(a=0.0,b=1.0,\mu=0.3260,\sigma=0.0500)$ &  $ 0.297 \pm 0.063 $  \\
Quadratic LD, $u_{{\rm TESS},1} $  & $\mathcal{N}_{\mathcal{U}}(a=0.0,b=1.0,\mu=0.2626,\sigma=0.0500)$ &  $ 0.229^{+0.087}_{-0.085} $  \\
Quadratic LD, $u_{{\rm Cheops},0} $  & $\mathcal{N}_{\mathcal{U}}(a=0.0,b=1.0,\mu=0.4436,\sigma=0.0500)$ &  $ 0.493 \pm 0.066 $  \\
Quadratic LD, $u_{{\rm Cheops},1} $  & $\mathcal{N}_{\mathcal{U}}(a=0.0,b=1.0,\mu=0.2329,\sigma=0.0500)$ &  $ 0.21 \pm 0.084 $  \\
RV mean, $\mu_{\rm Sophie}$ & $\mathcal{N}(\mu=-16077.1,\sigma=271.527)$ &  $ -16085.47 \pm 0.63 $  \\
RV mean, $\mu_{\rm HARPS-N}$ & $\mathcal{N}(\mu=-2.8479,\sigma=112.492)$ &  $ -14.1 \pm 0.34 $  \\
RV mean, $\mu_{\rm CAFE}$ & $\mathcal{N}(\mu=-16212.1,\sigma=77.5936)$ &  $ -16176.2 \pm 2.2 $  \\
quadratic RV trend term quadratic & $\mathcal{N}(\mu=0,\sigma=0.005)$ &  $ -4.95e-06 \pm 3.7e-07 $  \\
linear RV trend term linear & $\mathcal{N}(\mu=0,\sigma=0.05)$ &  $ -0.0667 \pm 0.001 $  \\
Log photometric scatter, $\log{\sigma_{{\rm TESS},s}/(\rm{ppt})}$  & $\mathcal{N}(\mu=0.1484,\sigma=3) $ &  $ -0.579 \pm 0.012 $  \\
Trend with normalised sine of roll angle, $df/d({\sin{\Phi}})_N$   & $\mathcal{N}(\mu=0,\sigma=1) $ &  $ -0.013 \pm 0.035 $  \\
Trend with normalised cosine of roll angle, $df/d({\cos{\Phi}})_N$   & $\mathcal{N}(\mu=0,\sigma=1) $ &  $ 0.062 \pm 0.025 $  \\
Trend with normalised background flux, $df/d({\cos{\Phi}})_N$   & $\mathcal{N}(\mu=0,\sigma=1) $ &  $ 0.68 \pm 0.91 $  \\
Mean flux, $\mu_{{\rm Cheops}}$ [ppt]  & $\mathcal{N}(\mu=0,\sigma=0.3127) $ &  $ 0.423 \pm 0.025 $  \\
Log photometric scatter, $\log{\sigma_{{\rm Cheops},s}/(\rm{ppt})}$  & $\mathcal{N}(\mu=-1.469,\sigma=3) $ &  $ -2.1^{+0.14}_{-0.18} $  \\


==> TOI1471_finalmodel_TOI1471_notessgp_norollangelgp_wpipe_nottvs_3rvpoly_noeccentricity_noldprior_20220824macro.tex <==
\newcommand{\TTeff}{ $ 5641 \pm 31 $ }
\newcommand{\TTeffshort}{ $ 5640 $ }

\newcommand{\TRs}{ $ 0.9622 \pm 0.0081 $ }
\newcommand{\TRsshort}{ $ 0.962 $ }

\newcommand{\Tg}{ $ 85.6^{+1.3}_{-2.2} $ }
\newcommand{\Tgshort}{ $ 86.0 $ }

\newcommand{\Tlogg}{ $ 4.45^{+0.015}_{-0.026} $ }
\newcommand{\Tloggshort}{ $ 4.45 $ }

\newcommand{\TKzero}{ $ 2.95 \pm 0.48 $ }
\newcommand{\TKzeroshort}{ $ 2.9 $ }

\newcommand{\TlogKzero}{ $ 1.08 \pm 0.17 $ }
\newcommand{\TlogKzeroshort}{ $ 1.1 $ }

\newcommand{\TKone}{ $ 1.25^{+0.44}_{-0.49} $ }
\newcommand{\TKoneshort}{ $ 1.2 $ }

\newcommand{\TlogKone}{ $ 0.22^{+0.3}_{-0.49} $ }
\newcommand{\TlogKoneshort}{ $ 0.2 $ }

\newcommand{\Ttzerozero}{ $ 1767.42088 \pm 0.00056 $ }
\newcommand{\Ttzerozeroshort}{ $ 1767.4209 $ }

\newcommand{\Ttzeroone}{ $ 1779.192 \pm 0.001 $ }
\newcommand{\Ttzerooneshort}{ $ 1779.192 $ }

\newcommand{\Tperiodzero}{ $ 20.772907 \pm 2.3\times10^{-5} $ }
\newcommand{\Tperiodzeroshort}{ $ 20.77291 $ }

\newcommand{\Tperiodone}{ $ 52.563518 \pm 7.1\times10^{-5} $ }
\newcommand{\Tperiodoneshort}{ $ 52.56352 $ }

\newcommand{\Trvoffsetszero}{ $ -16085.47 \pm 0.63 $ }
\newcommand{\Trvoffsetszeroshort}{ $ -16085.5 $ }

\newcommand{\Trvoffsetsone}{ $ -14.1 \pm 0.34 $ }
\newcommand{\Trvoffsetsoneshort}{ $ -14.1 $ }

\newcommand{\Trvoffsetstwo}{ $ -16176.2 \pm 2.2 $ }
\newcommand{\Trvoffsetstwoshort}{ $ -16176.0 $ }

\newcommand{\Trvtrendzero}{ $ -5\times10^{-6}^{+4\times10^{-7}}_{-3\times10^{-7}} $ }
\newcommand{\Trvtrendzeroshort}{ $ -5\times10^{-6} $ }

\newcommand{\Trvtrendone}{ $ -0.0667 \pm 0.001 $ }
\newcommand{\Trvtrendoneshort}{ $ -0.067 $ }

\newcommand{\Tsphot}{ $ 0.5607 \pm 0.0068 $ }
\newcommand{\Tsphotshort}{ $ 0.561 $ }

\newcommand{\Tlogsphot}{ $ -0.579 \pm 0.012 $ }
\newcommand{\Tlogsphotshort}{ $ -0.58 $ }

\newcommand{\Tdfdsinrollanglezero}{ $ -0.013 \pm 0.035 $ }
\newcommand{\Tdfdsinrollanglezeroshort}{ $ -0.01 $ }

\newcommand{\Tdfdcosrollanglezero}{ $ 0.062 \pm 0.025 $ }
\newcommand{\Tdfdcosrollanglezeroshort}{ $ 0.06 $ }

\newcommand{\Tdfdbgzero}{ $ 0.68 \pm 0.91 $ }
\newcommand{\Tdfdbgzeroshort}{ $ 0.7 $ }

\newcommand{\Tcheopsmeanzero}{ $ 0.423 \pm 0.025 $ }
\newcommand{\Tcheopsmeanzeroshort}{ $ 0.42 $ }

\newcommand{\Tscheops}{ $ 0.122 \pm 0.019 $ }
\newcommand{\Tscheopsshort}{ $ 0.12 $ }

\newcommand{\Tlogscheops}{ $ -2.1^{+0.14}_{-0.18} $ }
\newcommand{\Tlogscheopsshort}{ $ -2.1 $ }

\newcommand{\TMs}{ $ 1.012^{+0.044}_{-0.062} $ }
\newcommand{\TMsshort}{ $ 1.01 $ }

\newcommand{\Trorzero}{ $ 0.03706 \pm 0.00038 $ }
\newcommand{\Trorzeroshort}{ $ 0.0371 $ }

\newcommand{\Tlogrorzero}{ $ -3.295 \pm 0.01 $ }
\newcommand{\Tlogrorzeroshort}{ $ -3.3 $ }

\newcommand{\Trorone}{ $ 0.0318 \pm 0.00034 $ }
\newcommand{\Troroneshort}{ $ 0.0318 $ }

\newcommand{\Tlogrorone}{ $ -3.448 \pm 0.011 $ }
\newcommand{\Tlogroroneshort}{ $ -3.45 $ }

\newcommand{\Trplzero}{ $ 3.89 \pm 0.05 $ }
\newcommand{\Trplzeroshort}{ $ 3.89 $ }

\newcommand{\Trplone}{ $ 3.34 \pm 0.05 $ }
\newcommand{\Trploneshort}{ $ 3.34 $ }

\newcommand{\Tbzero}{ $ 0.12 \pm 0.1 $ }
\newcommand{\Tbzeroshort}{ $ 0.1 $ }

\newcommand{\Tbone}{ $ 0.233^{+0.07}_{-0.058} $ }
\newcommand{\Tboneshort}{ $ 0.23 $ }

\newcommand{\Tustartesszero}{ $ 0.297 \pm 0.063 $ }
\newcommand{\Tustartesszeroshort}{ $ 0.3 $ }

\newcommand{\Tustartessone}{ $ 0.229^{+0.087}_{-0.085} $ }
\newcommand{\Tustartessoneshort}{ $ 0.23 $ }

\newcommand{\Tustarcheopszero}{ $ 0.493 \pm 0.066 $ }
\newcommand{\Tustarcheopszeroshort}{ $ 0.49 $ }

\newcommand{\Tustarcheopsone}{ $ 0.21 \pm 0.084 $ }
\newcommand{\Tustarcheopsoneshort}{ $ 0.21 $ }

\newcommand{\TMpzero}{ $ 12.7 \pm 2.1 $ }
\newcommand{\TMpzeroshort}{ $ 13.0 $ }

\newcommand{\TMpone}{ $ 7.3 \pm 2.8 $ }
\newcommand{\TMponeshort}{ $ 7.0 $ }

\newcommand{\Trhopgcmthreezero}{ $ 1.19 \pm 0.2 $ }
\newcommand{\Trhopgcmthreezeroshort}{ $ 1.2 $ }

\newcommand{\Trhopgcmthreeone}{ $ 1.08 \pm 0.42 $ }
\newcommand{\Trhopgcmthreeoneshort}{ $ 1.1 $ }

\newcommand{\TaRszero}{ $ 31.93^{+0.46}_{-0.66} $ }
\newcommand{\TaRszeroshort}{ $ 31.9 $ }

\newcommand{\TaRsone}{ $ 59.3 \pm 1.0 $ }
\newcommand{\TaRsoneshort}{ $ 59.0 $ }

\newcommand{\Tsmazero}{ $ 0.1427^{+0.003}_{-0.0035} $ }
\newcommand{\Tsmazeroshort}{ $ 0.143 $ }

\newcommand{\Tsmaone}{ $ 0.265^{+0.0056}_{-0.0065} $ }
\newcommand{\Tsmaoneshort}{ $ 0.265 $ }

\newcommand{\TSinzero}{ $ 56400^{+2700}_{-2100} $ }
\newcommand{\TSinzeroshort}{ $ 56000 $ }

\newcommand{\TSinone}{ $ 16360^{+780}_{-600} $ }
\newcommand{\TSinoneshort}{ $ 16400 $ }

\newcommand{\TTsurfpzero}{ $ 667.8^{+7.8}_{-6.2} $ }
\newcommand{\TTsurfpzeroshort}{ $ 668.0 $ }

\newcommand{\TTsurfpone}{ $ 490.1^{+5.7}_{-4.5} $ }
\newcommand{\TTsurfponeshort}{ $ 490.0 $ }

\newcommand{\Ttdurzero}{ $ 0.2047^{+0.0015}_{-0.0015} $ }
\newcommand{\Ttdurzeroshort}{ $ 0.205 $ }

\newcommand{\Ttdurone}{ $ 0.2727 \pm 0.0013 $ }
\newcommand{\Ttduroneshort}{ $ 0.273 $ }

\newcommand{\TTSMzero}{ $ 103 \pm 18 $ }
\newcommand{\TTSMzeroshort}{ $ 100 $ }

\newcommand{\TTSMone}{ $ 83^{+56}_{-22} $ }
\newcommand{\TTSMoneshort}{ $ 80 $ }

\newcommand{\TTIC}{306263608}
\newcommand{\Tra}{30.9042722461231}
\newcommand{\Tdec}{21.2808637598307}
\newcommand{\THIP}{9618}
\newcommand{\TTYC}{1213-01071-1}
\newcommand{\TGAIA}{94468978202180352}
\newcommand{\Tcontratio}{0.000620889768}
\newcommand{\TTmag}{ $ 8.5725 \pm 0.006 $ }
\newcommand{\TTmagshort}{ $ 8.572 $ }

\newcommand{\TGAIAmag}{ $ 9.02543 \pm 0.00027 $ }
\newcommand{\TGAIAmagshort}{ $ 9.0254 $ }

\newcommand{\TVmag}{ $ 9.2 \pm 0.03 $ }
\newcommand{\TVmagshort}{ $ 9.2 $ }

\newcommand{\TJmag}{ $ 7.922 \pm 0.021 $ }
\newcommand{\TJmagshort}{ $ 7.92 $ }

\newcommand{\THmag}{ $ 7.656 \pm 0.036 $ }
\newcommand{\THmagshort}{ $ 7.66 $ }

\newcommand{\TKmag}{ $ 7.559 \pm 0.021 $ }
\newcommand{\TKmagshort}{ $ 7.56 $ }

\newcommand{\Twonemag}{ $ 7.489 \pm 0.034 $ }
\newcommand{\Twonemagshort}{ $ 7.49 $ }

\newcommand{\Twtwomag}{ $ 7.563 \pm 0.021 $ }
\newcommand{\Twtwomagshort}{ $ 7.56 $ }

\newcommand{\Twthreemag}{ $ 7.547 \pm 0.018 $ }
\newcommand{\Twthreemagshort}{ $ 7.55 $ }



==> TOI1471_newpipemodel_TOI1471_notessgp_norollangelgp_wrollanglespline_wpipe_nottvs_3rvpoly_2chetrend_weccentricity_wldprior_20230331macro.tex <==
\newcommand{\TTeff}{ $ 5604.0 \pm 27.0 $ }
\newcommand{\TTeffshort}{ $ 5600.0 $ }

\newcommand{\TRs}{ $ 0.9662 \pm 0.005 $ }
\newcommand{\TRsshort}{ $ 0.966 $ }

\newcommand{\Tg}{ $ 85.5^{+1.5}_{-3.3} $ }
\newcommand{\Tgshort}{ $ 85.0 $ }

\newcommand{\Tlogg}{ $ 4.448^{+0.017}_{-0.039} $ }
\newcommand{\Tloggshort}{ $ 4.45 $ }

\newcommand{\TdeltaImagcontam}{ $ 7.4 \pm 1.7 $ }
\newcommand{\TdeltaImagcontamshort}{ $ 7.0 $ }

\newcommand{\TdeltaVmagcontam}{ $ 9.0 \pm 2.0 $ }
\newcommand{\TdeltaVmagcontamshort}{ $ 9.0 $ }

\newcommand{\Ttzerozero}{ $ 1767.42088 \pm 0.00056 $ }
\newcommand{\Ttzerozeroshort}{ $ 1767.4209 $ }

\newcommand{\Ttzeroone}{ $ 1779.1919 \pm 0.001 $ }
\newcommand{\Ttzerooneshort}{ $ 1779.192 $ }

\newcommand{\Tperiodzero}{ $ 20.772906 \pm 2.3e-05 $ }
\newcommand{\Tperiodzeroshort}{ $ 20.77291 $ }

\newcommand{\Tperiodone}{ $ 52.563492 \pm 7.3e-05 $ }
\newcommand{\Tperiodoneshort}{ $ 52.56349 $ }

\newcommand{\Trvoffsetszero}{ $ -16082.51 \pm 0.63 $ }
\newcommand{\Trvoffsetszeroshort}{ $ -16082.5 $ }

\newcommand{\Trvoffsetsone}{ $ -11.28 \pm 0.34 $ }
\newcommand{\Trvoffsetsoneshort}{ $ -11.3 $ }

\newcommand{\Trvtrendzero}{ $ -5.3e-06^{+4e-07}_{-3e-07} $ }
\newcommand{\Trvtrendzeroshort}{ $ -5.3e-06 $ }

\newcommand{\Trvtrendone}{ $ -0.0671 \pm 0.001 $ }
\newcommand{\Trvtrendoneshort}{ $ -0.067 $ }

\newcommand{\Tsphot}{ $ 1.0^{+24.0}_{-1.0} $ }
\newcommand{\Tsphotshort}{ $ 0.0 $ }

\newcommand{\Tlogsphot}{ $ 0.2 \pm 2.9 $ }
\newcommand{\Tlogsphotshort}{ $ 0.0 $ }

\newcommand{\TdfdBG}{ $ -0.13 \pm 0.11 $ }
\newcommand{\TdfdBGshort}{ $ -0.1 $ }

\newcommand{\Tdfdsinrollangle}{ $ 0.004 \pm 0.043 $ }
\newcommand{\Tdfdsinrollangleshort}{ $ 0.0 $ }

\newcommand{\Tdfdcosrollangle}{ $ 0.119 \pm 0.043 $ }
\newcommand{\Tdfdcosrollangleshort}{ $ 0.12 $ }

\newcommand{\Tcheopsobspolytwozero}{ $ -0.049^{+0.046}_{-0.044} $ }
\newcommand{\Tcheopsobspolytwozeroshort}{ $ -0.05 $ }

\newcommand{\Tcheopsobspolytwoone}{ $ 0.01 \pm 0.13 $ }
\newcommand{\Tcheopsobspolytwooneshort}{ $ 0.0 $ }

\newcommand{\Tcheopsobspolythreezero}{ $ 0.01^{+0.035}_{-0.035} $ }
\newcommand{\Tcheopsobspolythreezeroshort}{ $ 0.01 $ }

\newcommand{\Tcheopsobspolythreeone}{ $ -0.02 \pm 0.13 $ }
\newcommand{\Tcheopsobspolythreeoneshort}{ $ -0.0 $ }

\newcommand{\Tcheopsobspolyfourzero}{ $ -0.133 \pm 0.039 $ }
\newcommand{\Tcheopsobspolyfourzeroshort}{ $ -0.13 $ }

\newcommand{\Tcheopsobspolyfourone}{ $ -0.02 \pm 0.13 $ }
\newcommand{\Tcheopsobspolyfouroneshort}{ $ -0.0 $ }

\newcommand{\Tcheopsobspolysixzero}{ $ -0.061 \pm 0.036 $ }
\newcommand{\Tcheopsobspolysixzeroshort}{ $ -0.06 $ }

\newcommand{\Tcheopsobspolysixone}{ $ -0.03 \pm 0.13 $ }
\newcommand{\Tcheopsobspolysixoneshort}{ $ -0.0 $ }

\newcommand{\Tscheops}{ $ 0.0005^{+0.0077}_{-0.0004} $ }
\newcommand{\Tscheopsshort}{ $ 0.0 $ }

\newcommand{\Tlogscheops}{ $ -7.7 \pm 2.9 $ }
\newcommand{\Tlogscheopsshort}{ $ -8.0 $ }

\newcommand{\Tsplineszero}{ $ -0.02 \pm 0.13 $ }
\newcommand{\Tsplineszeroshort}{ $ -0.0 $ }

\newcommand{\Tsplinesone}{ $ 0.166^{+0.096}_{-0.093} $ }
\newcommand{\Tsplinesoneshort}{ $ 0.17 $ }

\newcommand{\Tsplinestwo}{ $ 0.031 \pm 0.096 $ }
\newcommand{\Tsplinestwoshort}{ $ 0.03 $ }

\newcommand{\Tsplinesthree}{ $ 0.006 \pm 0.09 $ }
\newcommand{\Tsplinesthreeshort}{ $ 0.01 $ }

\newcommand{\Tsplinesfour}{ $ 0.039^{+0.088}_{-0.084} $ }
\newcommand{\Tsplinesfourshort}{ $ 0.04 $ }

\newcommand{\Tsplinesfive}{ $ -0.029 \pm 0.08 $ }
\newcommand{\Tsplinesfiveshort}{ $ -0.03 $ }

\newcommand{\Tsplinessix}{ $ 0.123 \pm 0.08 $ }
\newcommand{\Tsplinessixshort}{ $ 0.12 $ }

\newcommand{\Tsplinesseven}{ $ -0.118 \pm 0.078 $ }
\newcommand{\Tsplinessevenshort}{ $ -0.12 $ }

\newcommand{\Tsplineseight}{ $ -0.006 \pm 0.076 $ }
\newcommand{\Tsplineseightshort}{ $ -0.01 $ }

\newcommand{\Tsplinesnine}{ $ -0.151^{+0.077}_{-0.074} $ }
\newcommand{\Tsplinesnineshort}{ $ -0.15 $ }

\newcommand{\Tsplinesonezero}{ $ -0.136 \pm 0.072 $ }
\newcommand{\Tsplinesonezeroshort}{ $ -0.14 $ }

\newcommand{\Tsplinesoneone}{ $ -0.012 \pm 0.071 $ }
\newcommand{\Tsplinesoneoneshort}{ $ -0.01 $ }

\newcommand{\Tsplinesonetwo}{ $ -0.094 \pm 0.071 $ }
\newcommand{\Tsplinesonetwoshort}{ $ -0.09 $ }

\newcommand{\Tsplinesonethree}{ $ 0.073 \pm 0.07 $ }
\newcommand{\Tsplinesonethreeshort}{ $ 0.07 $ }

\newcommand{\Tsplinesonefour}{ $ 0.012 \pm 0.071 $ }
\newcommand{\Tsplinesonefourshort}{ $ 0.01 $ }

\newcommand{\Tsplinesonefive}{ $ 0.108 \pm 0.071 $ }
\newcommand{\Tsplinesonefiveshort}{ $ 0.11 $ }

\newcommand{\Tsplinesonesix}{ $ -0.092 \pm 0.074 $ }
\newcommand{\Tsplinesonesixshort}{ $ -0.09 $ }

\newcommand{\Tsplinesoneseven}{ $ 0.166 \pm 0.076 $ }
\newcommand{\Tsplinesonesevenshort}{ $ 0.17 $ }

\newcommand{\Tsplinesoneeight}{ $ -0.082 \pm 0.074 $ }
\newcommand{\Tsplinesoneeightshort}{ $ -0.08 $ }

\newcommand{\Tsplinesonenine}{ $ 0.016^{+0.076}_{-0.075} $ }
\newcommand{\Tsplinesonenineshort}{ $ 0.02 $ }

\newcommand{\Tsplinestwozero}{ $ 0.053^{+0.075}_{-0.076} $ }
\newcommand{\Tsplinestwozeroshort}{ $ 0.05 $ }

\newcommand{\Tsplinestwoone}{ $ -0.074 \pm 0.077 $ }
\newcommand{\Tsplinestwooneshort}{ $ -0.07 $ }

\newcommand{\Tsplinestwotwo}{ $ 0.111 \pm 0.083 $ }
\newcommand{\Tsplinestwotwoshort}{ $ 0.11 $ }

\newcommand{\Tsplinestwothree}{ $ -0.157 \pm 0.093 $ }
\newcommand{\Tsplinestwothreeshort}{ $ -0.16 $ }

\newcommand{\Tsplinestwofour}{ $ 0.22 \pm 0.1 $ }
\newcommand{\Tsplinestwofourshort}{ $ 0.2 $ }

\newcommand{\Tsplinestwofive}{ $ -0.21 \pm 0.11 $ }
\newcommand{\Tsplinestwofiveshort}{ $ -0.2 $ }

\newcommand{\TMs}{ $ 1.018^{+0.046}_{-0.086} $ }
\newcommand{\TMsshort}{ $ 1.02 $ }

\newcommand{\Ttessmult}{ $ 1.0011^{+0.004}_{-0.0009} $ }
\newcommand{\Ttessmultshort}{ $ 1.001 $ }

\newcommand{\Tcheopsmult}{ $ 1.0003^{+0.0014}_{-0.0002} $ }
\newcommand{\Tcheopsmultshort}{ $ 1.0 $ }

\newcommand{\Trorzero}{ $ 0.03702 \pm 0.00037 $ }
\newcommand{\Trorzeroshort}{ $ 0.037 $ }

\newcommand{\Tlogrorzero}{ $ -3.296 \pm 0.01 $ }
\newcommand{\Tlogrorzeroshort}{ $ -3.3 $ }

\newcommand{\Trorone}{ $ 0.03175^{+0.00035}_{-0.00033} $ }
\newcommand{\Troroneshort}{ $ 0.0318 $ }

\newcommand{\Tlogrorone}{ $ -3.45 \pm 0.011 $ }
\newcommand{\Tlogroroneshort}{ $ -3.45 $ }

\newcommand{\Trplzero}{ $ 3.901 \pm 0.044 $ }
\newcommand{\Trplzeroshort}{ $ 3.9 $ }

\newcommand{\Trplone}{ $ 3.347 \pm 0.04 $ }
\newcommand{\Trploneshort}{ $ 3.35 $ }

\newcommand{\Tbzero}{ $ 0.14 \pm 0.12 $ }
\newcommand{\Tbzeroshort}{ $ 0.1 $ }

\newcommand{\Tbone}{ $ 0.239^{+0.096}_{-0.066} $ }
\newcommand{\Tboneshort}{ $ 0.24 $ }

\newcommand{\TKzero}{ $ 3.51 \pm 0.48 $ }
\newcommand{\TKzeroshort}{ $ 3.5 $ }

\newcommand{\TKone}{ $ 1.03 \pm 0.42 $ }
\newcommand{\TKoneshort}{ $ 1.0 $ }

\newcommand{\Tustartesszero}{ $ 0.302 \pm 0.062 $ }
\newcommand{\Tustartesszeroshort}{ $ 0.3 $ }

\newcommand{\Tustartessone}{ $ 0.22 \pm 0.088 $ }
\newcommand{\Tustartessoneshort}{ $ 0.22 $ }

\newcommand{\Tustarcheopszero}{ $ 0.501 \pm 0.062 $ }
\newcommand{\Tustarcheopszeroshort}{ $ 0.5 $ }

\newcommand{\Tustarcheopsone}{ $ 0.174 \pm 0.082 $ }
\newcommand{\Tustarcheopsoneshort}{ $ 0.17 $ }

\newcommand{\Teccalpha}{ $ 1.12 \pm 0.1 $ }
\newcommand{\Teccalphashort}{ $ 1.1 $ }

\newcommand{\Teccbeta}{ $ 3.09 \pm 0.3 $ }
\newcommand{\Teccbetashort}{ $ 3.1 $ }

\newcommand{\Tecczero}{ $ 0.22 \pm 0.2 $ }
\newcommand{\Tecczeroshort}{ $ 0.2 $ }

\newcommand{\Teccone}{ $ 0.22^{+0.25}_{-0.16} $ }
\newcommand{\Tecconeshort}{ $ 0.2 $ }

\newcommand{\Tomegazero}{ $ 0.3 \pm 2.1 $ }
\newcommand{\Tomegazeroshort}{ $ 0.0 $ }

\newcommand{\Tomegaone}{ $ 0.1 \pm 2.2 $ }
\newcommand{\Tomegaoneshort}{ $ 0.0 $ }

\newcommand{\TMpzero}{ $ 14.3 \pm 2.4 $ }
\newcommand{\TMpzeroshort}{ $ 14.0 $ }

\newcommand{\TMpone}{ $ 13.11 $ }
\newcommand{\TMponeshort}{ $ 13.1 $ }

\newcommand{\Trhopgcmthreezero}{ $ 1.33 \pm 0.23 $ }
\newcommand{\Trhopgcmthreezeroshort}{ $ 1.3 $ }

\newcommand{\Trhopgcmthreeone}{ $ 0.83 \pm 0.36 $ }
\newcommand{\Trhopgcmthreeoneshort}{ $ 0.8 $ }

\newcommand{\TaRszero}{ $ 31.99^{+0.48}_{-0.92} $ }
\newcommand{\TaRszeroshort}{ $ 32.0 $ }

\newcommand{\TaRsone}{ $ 59.4^{+0.9}_{-1.7} $ }
\newcommand{\TaRsoneshort}{ $ 59.0 $ }

\newcommand{\Tsmazero}{ $ 0.1435^{+0.0026}_{-0.0041} $ }
\newcommand{\Tsmazeroshort}{ $ 0.144 $ }

\newcommand{\Tsmaone}{ $ 0.2665^{+0.0049}_{-0.0076} $ }
\newcommand{\Tsmaoneshort}{ $ 0.266 $ }

\newcommand{\TSinzero}{ $ 54800^{+3300}_{-2000} $ }
\newcommand{\TSinzeroshort}{ $ 55000.0 $ }

\newcommand{\TSinone}{ $ 15900^{+970}_{-590} $ }
\newcommand{\TSinoneshort}{ $ 15900.0 $ }

\newcommand{\TTsurfpzero}{ $ 663.1^{+9.9}_{-6.3} $ }
\newcommand{\TTsurfpzeroshort}{ $ 663.0 $ }

\newcommand{\TTsurfpone}{ $ 486.6^{+7.3}_{-4.6} $ }
\newcommand{\TTsurfponeshort}{ $ 487.0 $ }

\newcommand{\Ttdurzero}{ $ 0.2047^{+0.0015}_{-0.0014} $ }
\newcommand{\Ttdurzeroshort}{ $ 0.205 $ }

\newcommand{\Ttdurone}{ $ 0.2731 \pm 0.0012 $ }
\newcommand{\Ttduroneshort}{ $ 0.273 $ }

\newcommand{\TTSMzero}{ $ 117.0^{+26.0}_{-17.0} $ }
\newcommand{\TTSMzeroshort}{ $ 120.0 $ }

\newcommand{\TTSMone}{ $ 58.7 $ }
\newcommand{\TTSMoneshort}{ $ 59.0 $ }

\newcommand{\TTIC}{306263608}
\newcommand{\THIP}{9618}
\newcommand{\TTYC}{1213-01071-1}
\newcommand{\TGAIA}{94468978202180352}
\newcommand{\Tra}{30.904272}
\newcommand{\Tdec}{21.280864}
\newcommand{\Tcontratio}{0.000621}
\newcommand{\TTmag}{ $ 8.5725 \pm 0.006 $ }
\newcommand{\TTmagshort}{ $ 8.572 $ }

\newcommand{\TGAIAmag}{ $ 9.02543 \pm 0.00027 $ }
\newcommand{\TGAIAmagshort}{ $ 9.0254 $ }

\newcommand{\TVmag}{ $ 9.2 \pm 0.03 $ }
\newcommand{\TVmagshort}{ $ 9.2 $ }

\newcommand{\TJmag}{ $ 7.922 \pm 0.021 $ }
\newcommand{\TJmagshort}{ $ 7.92 $ }

\newcommand{\THmag}{ $ 7.656 \pm 0.036 $ }
\newcommand{\THmagshort}{ $ 7.66 $ }

\newcommand{\TKmag}{ $ 7.559 \pm 0.021 $ }
\newcommand{\TKmagshort}{ $ 7.56 $ }

\newcommand{\Twonemag}{ $ 7.489 \pm 0.034 $ }
\newcommand{\Twonemagshort}{ $ 7.49 $ }

\newcommand{\Twtwomag}{ $ 7.563 \pm 0.021 $ }
\newcommand{\Twtwomagshort}{ $ 7.56 $ }

\newcommand{\Twthreemag}{ $ 7.547 \pm 0.018 $ }
\newcommand{\Twthreemagshort}{ $ 7.55 $ }



==> TOI1471_newpipemodel_macro.tex <==
\newcommand{\TTeff}{ $ 5604.0 \pm 27.0 $ }
\newcommand{\TTeffshort}{ $ 5600.0 $ }

\newcommand{\TRs}{ $ 0.9662 \pm 0.005 $ }
\newcommand{\TRsshort}{ $ 0.966 $ }

\newcommand{\Tg}{ $ 85.5^{+1.5}_{-3.3} $ }
\newcommand{\Tgshort}{ $ 85.0 $ }

\newcommand{\Tlogg}{ $ 4.448^{+0.017}_{-0.039} $ }
\newcommand{\Tloggshort}{ $ 4.45 $ }

\newcommand{\TdeltaImagcontam}{ $ 7.4 \pm 1.7 $ }
\newcommand{\TdeltaImagcontamshort}{ $ 7.0 $ }

\newcommand{\TdeltaVmagcontam}{ $ 9.0 \pm 2.0 $ }
\newcommand{\TdeltaVmagcontamshort}{ $ 9.0 $ }

\newcommand{\Ttzerozero}{ $ 1767.42088 \pm 0.00056 $ }
\newcommand{\Ttzerozeroshort}{ $ 1767.4209 $ }

\newcommand{\Ttzeroone}{ $ 1779.1919 \pm 0.001 $ }
\newcommand{\Ttzerooneshort}{ $ 1779.192 $ }

\newcommand{\Tperiodzero}{ $ 20.772906 \pm 2.3e-05 $ }
\newcommand{\Tperiodzeroshort}{ $ 20.77291 $ }

\newcommand{\Tperiodone}{ $ 52.563492 \pm 7.3e-05 $ }
\newcommand{\Tperiodoneshort}{ $ 52.56349 $ }

\newcommand{\Trvoffsetszero}{ $ -16082.51 \pm 0.63 $ }
\newcommand{\Trvoffsetszeroshort}{ $ -16082.5 $ }

\newcommand{\Trvoffsetsone}{ $ -11.28 \pm 0.34 $ }
\newcommand{\Trvoffsetsoneshort}{ $ -11.3 $ }

\newcommand{\Trvtrendzero}{ $ -5.3e-06^{+4e-07}_{-3e-07} $ }
\newcommand{\Trvtrendzeroshort}{ $ -5.3e-06 $ }

\newcommand{\Trvtrendone}{ $ -0.0671 \pm 0.001 $ }
\newcommand{\Trvtrendoneshort}{ $ -0.067 $ }

\newcommand{\Tsphot}{ $ 1.0^{+24.0}_{-1.0} $ }
\newcommand{\Tsphotshort}{ $ 0.0 $ }

\newcommand{\Tlogsphot}{ $ 0.2 \pm 2.9 $ }
\newcommand{\Tlogsphotshort}{ $ 0.0 $ }

\newcommand{\TdfdBG}{ $ -0.13 \pm 0.11 $ }
\newcommand{\TdfdBGshort}{ $ -0.1 $ }

\newcommand{\Tdfdsinrollangle}{ $ 0.004 \pm 0.043 $ }
\newcommand{\Tdfdsinrollangleshort}{ $ 0.0 $ }

\newcommand{\Tdfdcosrollangle}{ $ 0.119 \pm 0.043 $ }
\newcommand{\Tdfdcosrollangleshort}{ $ 0.12 $ }

\newcommand{\Tcheopsobspolytwozero}{ $ -0.049^{+0.046}_{-0.044} $ }
\newcommand{\Tcheopsobspolytwozeroshort}{ $ -0.05 $ }

\newcommand{\Tcheopsobspolytwoone}{ $ 0.01 \pm 0.13 $ }
\newcommand{\Tcheopsobspolytwooneshort}{ $ 0.0 $ }

\newcommand{\Tcheopsobspolythreezero}{ $ 0.01^{+0.035}_{-0.035} $ }
\newcommand{\Tcheopsobspolythreezeroshort}{ $ 0.01 $ }

\newcommand{\Tcheopsobspolythreeone}{ $ -0.02 \pm 0.13 $ }
\newcommand{\Tcheopsobspolythreeoneshort}{ $ -0.0 $ }

\newcommand{\Tcheopsobspolyfourzero}{ $ -0.133 \pm 0.039 $ }
\newcommand{\Tcheopsobspolyfourzeroshort}{ $ -0.13 $ }

\newcommand{\Tcheopsobspolyfourone}{ $ -0.02 \pm 0.13 $ }
\newcommand{\Tcheopsobspolyfouroneshort}{ $ -0.0 $ }

\newcommand{\Tcheopsobspolysixzero}{ $ -0.061 \pm 0.036 $ }
\newcommand{\Tcheopsobspolysixzeroshort}{ $ -0.06 $ }

\newcommand{\Tcheopsobspolysixone}{ $ -0.03 \pm 0.13 $ }
\newcommand{\Tcheopsobspolysixoneshort}{ $ -0.0 $ }

\newcommand{\Tscheops}{ $ 0.0005^{+0.0077}_{-0.0004} $ }
\newcommand{\Tscheopsshort}{ $ 0.0 $ }

\newcommand{\Tlogscheops}{ $ -7.7 \pm 2.9 $ }
\newcommand{\Tlogscheopsshort}{ $ -8.0 $ }

\newcommand{\Tsplineszero}{ $ -0.02 \pm 0.13 $ }
\newcommand{\Tsplineszeroshort}{ $ -0.0 $ }

\newcommand{\Tsplinesone}{ $ 0.166^{+0.096}_{-0.093} $ }
\newcommand{\Tsplinesoneshort}{ $ 0.17 $ }

\newcommand{\Tsplinestwo}{ $ 0.031 \pm 0.096 $ }
\newcommand{\Tsplinestwoshort}{ $ 0.03 $ }

\newcommand{\Tsplinesthree}{ $ 0.006 \pm 0.09 $ }
\newcommand{\Tsplinesthreeshort}{ $ 0.01 $ }

\newcommand{\Tsplinesfour}{ $ 0.039^{+0.088}_{-0.084} $ }
\newcommand{\Tsplinesfourshort}{ $ 0.04 $ }

\newcommand{\Tsplinesfive}{ $ -0.029 \pm 0.08 $ }
\newcommand{\Tsplinesfiveshort}{ $ -0.03 $ }

\newcommand{\Tsplinessix}{ $ 0.123 \pm 0.08 $ }
\newcommand{\Tsplinessixshort}{ $ 0.12 $ }

\newcommand{\Tsplinesseven}{ $ -0.118 \pm 0.078 $ }
\newcommand{\Tsplinessevenshort}{ $ -0.12 $ }

\newcommand{\Tsplineseight}{ $ -0.006 \pm 0.076 $ }
\newcommand{\Tsplineseightshort}{ $ -0.01 $ }

\newcommand{\Tsplinesnine}{ $ -0.151^{+0.077}_{-0.074} $ }
\newcommand{\Tsplinesnineshort}{ $ -0.15 $ }

\newcommand{\Tsplinesonezero}{ $ -0.136 \pm 0.072 $ }
\newcommand{\Tsplinesonezeroshort}{ $ -0.14 $ }

\newcommand{\Tsplinesoneone}{ $ -0.012 \pm 0.071 $ }
\newcommand{\Tsplinesoneoneshort}{ $ -0.01 $ }

\newcommand{\Tsplinesonetwo}{ $ -0.094 \pm 0.071 $ }
\newcommand{\Tsplinesonetwoshort}{ $ -0.09 $ }

\newcommand{\Tsplinesonethree}{ $ 0.073 \pm 0.07 $ }
\newcommand{\Tsplinesonethreeshort}{ $ 0.07 $ }

\newcommand{\Tsplinesonefour}{ $ 0.012 \pm 0.071 $ }
\newcommand{\Tsplinesonefourshort}{ $ 0.01 $ }

\newcommand{\Tsplinesonefive}{ $ 0.108 \pm 0.071 $ }
\newcommand{\Tsplinesonefiveshort}{ $ 0.11 $ }

\newcommand{\Tsplinesonesix}{ $ -0.092 \pm 0.074 $ }
\newcommand{\Tsplinesonesixshort}{ $ -0.09 $ }

\newcommand{\Tsplinesoneseven}{ $ 0.166 \pm 0.076 $ }
\newcommand{\Tsplinesonesevenshort}{ $ 0.17 $ }

\newcommand{\Tsplinesoneeight}{ $ -0.082 \pm 0.074 $ }
\newcommand{\Tsplinesoneeightshort}{ $ -0.08 $ }

\newcommand{\Tsplinesonenine}{ $ 0.016^{+0.076}_{-0.075} $ }
\newcommand{\Tsplinesonenineshort}{ $ 0.02 $ }

\newcommand{\Tsplinestwozero}{ $ 0.053^{+0.075}_{-0.076} $ }
\newcommand{\Tsplinestwozeroshort}{ $ 0.05 $ }

\newcommand{\Tsplinestwoone}{ $ -0.074 \pm 0.077 $ }
\newcommand{\Tsplinestwooneshort}{ $ -0.07 $ }

\newcommand{\Tsplinestwotwo}{ $ 0.111 \pm 0.083 $ }
\newcommand{\Tsplinestwotwoshort}{ $ 0.11 $ }

\newcommand{\Tsplinestwothree}{ $ -0.157 \pm 0.093 $ }
\newcommand{\Tsplinestwothreeshort}{ $ -0.16 $ }

\newcommand{\Tsplinestwofour}{ $ 0.22 \pm 0.1 $ }
\newcommand{\Tsplinestwofourshort}{ $ 0.2 $ }

\newcommand{\Tsplinestwofive}{ $ -0.21 \pm 0.11 $ }
\newcommand{\Tsplinestwofiveshort}{ $ -0.2 $ }

\newcommand{\TMs}{ $ 1.018^{+0.046}_{-0.086} $ }
\newcommand{\TMsshort}{ $ 1.02 $ }

\newcommand{\Ttessmult}{ $ 1.0011^{+0.004}_{-0.0009} $ }
\newcommand{\Ttessmultshort}{ $ 1.001 $ }

\newcommand{\Tcheopsmult}{ $ 1.0003^{+0.0014}_{-0.0002} $ }
\newcommand{\Tcheopsmultshort}{ $ 1.0 $ }

\newcommand{\Trorzero}{ $ 0.03702 \pm 0.00037 $ }
\newcommand{\Trorzeroshort}{ $ 0.037 $ }

\newcommand{\Tlogrorzero}{ $ -3.296 \pm 0.01 $ }
\newcommand{\Tlogrorzeroshort}{ $ -3.3 $ }

\newcommand{\Trorone}{ $ 0.03175^{+0.00035}_{-0.00033} $ }
\newcommand{\Troroneshort}{ $ 0.0318 $ }

\newcommand{\Tlogrorone}{ $ -3.45 \pm 0.011 $ }
\newcommand{\Tlogroroneshort}{ $ -3.45 $ }

\newcommand{\Trplzero}{ $ 3.901 \pm 0.044 $ }
\newcommand{\Trplzeroshort}{ $ 3.9 $ }

\newcommand{\Trplone}{ $ 3.347 \pm 0.04 $ }
\newcommand{\Trploneshort}{ $ 3.35 $ }

\newcommand{\Tbzero}{ $ 0.14 \pm 0.12 $ }
\newcommand{\Tbzeroshort}{ $ 0.1 $ }

\newcommand{\Tbone}{ $ 0.239^{+0.096}_{-0.066} $ }
\newcommand{\Tboneshort}{ $ 0.24 $ }

\newcommand{\TKzero}{ $ 3.51 \pm 0.48 $ }
\newcommand{\TKzeroshort}{ $ 3.5 $ }

\newcommand{\TKone}{ $ 1.03 \pm 0.42 $ }
\newcommand{\TKoneshort}{ $ 1.0 $ }

\newcommand{\Tustartesszero}{ $ 0.302 \pm 0.062 $ }
\newcommand{\Tustartesszeroshort}{ $ 0.3 $ }

\newcommand{\Tustartessone}{ $ 0.22 \pm 0.088 $ }
\newcommand{\Tustartessoneshort}{ $ 0.22 $ }

\newcommand{\Tustarcheopszero}{ $ 0.501 \pm 0.062 $ }
\newcommand{\Tustarcheopszeroshort}{ $ 0.5 $ }

\newcommand{\Tustarcheopsone}{ $ 0.174 \pm 0.082 $ }
\newcommand{\Tustarcheopsoneshort}{ $ 0.17 $ }

\newcommand{\Teccalpha}{ $ 1.12 \pm 0.1 $ }
\newcommand{\Teccalphashort}{ $ 1.1 $ }

\newcommand{\Teccbeta}{ $ 3.09 \pm 0.3 $ }
\newcommand{\Teccbetashort}{ $ 3.1 $ }

\newcommand{\Tecczero}{ $ 0.22 \pm 0.2 $ }
\newcommand{\Tecczeroshort}{ $ 0.2 $ }

\newcommand{\Teccone}{ $ 0.22^{+0.25}_{-0.16} $ }
\newcommand{\Tecconeshort}{ $ 0.2 $ }

\newcommand{\Tomegazero}{ $ 0.3 \pm 2.1 $ }
\newcommand{\Tomegazeroshort}{ $ 0.0 $ }

\newcommand{\Tomegaone}{ $ 0.1 \pm 2.2 $ }
\newcommand{\Tomegaoneshort}{ $ 0.0 $ }

\newcommand{\TMpzero}{ $ 14.3 \pm 2.4 $ }
\newcommand{\TMpzeroshort}{ $ 14.0 $ }

\newcommand{\TMpone}{ $ 13.11 $ }
\newcommand{\TMponeshort}{ $ 13.1 $ }

\newcommand{\Trhopgcmthreezero}{ $ 1.33 \pm 0.23 $ }
\newcommand{\Trhopgcmthreezeroshort}{ $ 1.3 $ }

\newcommand{\Trhopgcmthreeone}{ $ 0.83 \pm 0.36 $ }
\newcommand{\Trhopgcmthreeoneshort}{ $ 0.8 $ }

\newcommand{\TaRszero}{ $ 31.99^{+0.48}_{-0.92} $ }
\newcommand{\TaRszeroshort}{ $ 32.0 $ }

\newcommand{\TaRsone}{ $ 59.4^{+0.9}_{-1.7} $ }
\newcommand{\TaRsoneshort}{ $ 59.0 $ }

\newcommand{\Tsmazero}{ $ 0.1435^{+0.0026}_{-0.0041} $ }
\newcommand{\Tsmazeroshort}{ $ 0.144 $ }

\newcommand{\Tsmaone}{ $ 0.2665^{+0.0049}_{-0.0076} $ }
\newcommand{\Tsmaoneshort}{ $ 0.266 $ }

\newcommand{\TSinzero}{ $ 54800^{+3300}_{-2000} $ }
\newcommand{\TSinzeroshort}{ $ 55000.0 $ }

\newcommand{\TSinone}{ $ 15900^{+970}_{-590} $ }
\newcommand{\TSinoneshort}{ $ 15900.0 $ }

\newcommand{\TTsurfpzero}{ $ 663.1^{+9.9}_{-6.3} $ }
\newcommand{\TTsurfpzeroshort}{ $ 663.0 $ }

\newcommand{\TTsurfpone}{ $ 486.6^{+7.3}_{-4.6} $ }
\newcommand{\TTsurfponeshort}{ $ 487.0 $ }

\newcommand{\Ttdurzero}{ $ 0.2047^{+0.0015}_{-0.0014} $ }
\newcommand{\Ttdurzeroshort}{ $ 0.205 $ }

\newcommand{\Ttdurone}{ $ 0.2731 \pm 0.0012 $ }
\newcommand{\Ttduroneshort}{ $ 0.273 $ }

\newcommand{\TTSMzero}{ $ 117.0^{+26.0}_{-17.0} $ }
\newcommand{\TTSMzeroshort}{ $ 120.0 $ }

\newcommand{\TTSMone}{ $ 58.7 $ }
\newcommand{\TTSMoneshort}{ $ 59.0 $ }

\newcommand{\TTIC}{306263608}
\newcommand{\THIP}{9618}
\newcommand{\TTYC}{1213-01071-1}
\newcommand{\TGAIA}{94468978202180352}
\newcommand{\Tra}{30.904272}
\newcommand{\Tdec}{21.280864}
\newcommand{\Tcontratio}{0.000621}
\newcommand{\TTmag}{ $ 8.5725 \pm 0.006 $ }
\newcommand{\TTmagshort}{ $ 8.572 $ }

\newcommand{\TGAIAmag}{ $ 9.02543 \pm 0.00027 $ }
\newcommand{\TGAIAmagshort}{ $ 9.0254 $ }

\newcommand{\TVmag}{ $ 9.2 \pm 0.03 $ }
\newcommand{\TVmagshort}{ $ 9.2 $ }

\newcommand{\TJmag}{ $ 7.922 \pm 0.021 $ }
\newcommand{\TJmagshort}{ $ 7.92 $ }

\newcommand{\THmag}{ $ 7.656 \pm 0.036 $ }
\newcommand{\THmagshort}{ $ 7.66 $ }

\newcommand{\TKmag}{ $ 7.559 \pm 0.021 $ }
\newcommand{\TKmagshort}{ $ 7.56 $ }

\newcommand{\Twonemag}{ $ 7.489 \pm 0.034 $ }
\newcommand{\Twonemagshort}{ $ 7.49 $ }

\newcommand{\Twtwomag}{ $ 7.563 \pm 0.021 $ }
\newcommand{\Twtwomagshort}{ $ 7.56 $ }

\newcommand{\Twthreemag}{ $ 7.547 \pm 0.018 $ }
\newcommand{\Twthreemagshort}{ $ 7.55 $ }



==> TOI1471_newpipemodel_modeltable1.tex <==
Stellar temperature, \teff{}  [K]  & $\mathcal{N}(\mu=5610,\sigma=30) $ &  $ 5604.0 \pm 27.0 $  \\
Stellar radius, $R_s$ [$R_\oplus$] & $\mathcal{N}(\mu=0.9662,\sigma=0.005) $ &  $ 0.9662 \pm 0.005 $  \\
log stellar surface gravity, \logg{}  [cgs] & $\mathcal{N}(\mu=4.47,\sigma=0.1) $ &  $ 4.448^{+0.017}_{-0.039} $  \\
I mag contamination from companion, $\Delta I$  & $\mathcal{N}(\mu=7.398,\sigma=1.767) $ &  $ 7.4 \pm 1.7 $  \\
V mag contamination from companion, $\Delta V$  & $\mathcal{N}(\mu=8.966,\sigma=2.076) $ &  $ 9.0 \pm 2.0 $  \\
Quadratic LD, $u_{{\rm TESS},0} $  & $\mathcal{N}_{\mathcal{U}}(a=0.0,b=1.0,\mu=0.3304,\sigma=0.0500)$ &  $ 0.302 \pm 0.062 $  \\
Quadratic LD, $u_{{\rm TESS},1} $  & $\mathcal{N}_{\mathcal{U}}(a=0.0,b=1.0,\mu=0.2603,\sigma=0.0500)$ &  $ 0.22 \pm 0.088 $  \\
Quadratic LD, $u_{{\rm Cheops},0} $  & $\mathcal{N}_{\mathcal{U}}(a=0.0,b=1.0,\mu=0.4499,\sigma=0.0500)$ &  $ 0.501 \pm 0.062 $  \\
Quadratic LD, $u_{{\rm Cheops},1} $  & $\mathcal{N}_{\mathcal{U}}(a=0.0,b=1.0,\mu=0.2289,\sigma=0.0500)$ &  $ 0.174 \pm 0.082 $  \\
Eccentricity & $\Beta(\alpha=0.867, \beta=3.03)^{\ddagger}$ &  $ 0.22 \pm 0.2 $  \\
Eccentricity & $\Beta(\alpha=0.867, \beta=3.03)^{\ddagger}$ &  $ 0.22^{+0.25}_{-0.16} $  \\
Argument of periasteron & $\mathcal{{U}}(a=-\pi,b=\pi)$ &  $ 0.5 \pm 3.9 $  \\
Argument of periasteron & $\mathcal{{U}}(a=-\pi,b=\pi)$ &  $ -0.1 \pm 3.9 $  \\
RV mean, $\mu_{\rm Sophie}$ & $\mathcal{N}(\mu=-16077.1,\sigma=271.527)$ &  $ -16082.51 \pm 0.63 $  \\
RV mean, $\mu_{\rm HARPS-N}$ & $\mathcal{N}(\mu=-2.8479,\sigma=112.492)$ &  $ -11.28 \pm 0.34 $  \\
quadratic RV trend term quadratic & $\mathcal{N}(\mu=0,\sigma=0.005)$ &  $ -5.27e-06 \pm 3.8e-07 $  \\
linear RV trend term linear & $\mathcal{N}(\mu=0,\sigma=0.05)$ &  $ -0.0671 \pm 0.001 $  \\
Log photometric scatter, $\log{\sigma_{{\rm TESS},s}/(\rm{ppt})}$  & $\mathcal{N}(\mu=0.1435,\sigma=3) $ &  $ 0.2 \pm 2.9 $  \\
Trend with normalised background flux, $df/d({\cos{\Phi}})_N$   & $\mathcal{N}(\mu=0,\sigma=0.3819) $ &  $ -0.13 \pm 0.11 $  \\
Trend with normalised sine of roll angle, $df/d({\sin{\Phi}})_N$   & $\mathcal{N}(\mu=0,\sigma=0.3819) $ &  $ 0.004 \pm 0.043 $  \\
Trend with normalised cosine of roll angle, $df/d({\cos{\Phi}})_N$   & $\mathcal{N}(\mu=0,\sigma=0.3819) $ &  $ 0.119 \pm 0.043 $  \\
fk=PR110048_TG017201_V0200 flux trend polynomial 0 & $\mathcal{N}(\mu=0,\sigma=0.852144)$ &  $ -0.049^{+0.046}_{-0.044} $  \\
fk=PR110048_TG017201_V0200 flux trend polynomial 1 & $\mathcal{N}(\mu=0,\sigma=0.313486)$ &  $ 0.01 \pm 0.13 $  \\
fk=PR110048_TG017301_V0200 flux trend polynomial 0 & $\mathcal{N}(\mu=0,\sigma=0.852144)$ &  $ 0.01^{+0.035}_{-0.035} $  \\
fk=PR110048_TG017301_V0200 flux trend polynomial 1 & $\mathcal{N}(\mu=0,\sigma=0.313486)$ &  $ -0.02 \pm 0.13 $  \\
fk=PR110048_TG017401_V0200 flux trend polynomial 0 & $\mathcal{N}(\mu=0,\sigma=0.852144)$ &  $ -0.133 \pm 0.039 $  \\
fk=PR110048_TG017401_V0200 flux trend polynomial 1 & $\mathcal{N}(\mu=0,\sigma=0.313486)$ &  $ -0.02 \pm 0.13 $  \\
fk=PR110048_TG017601_V0200 flux trend polynomial 0 & $\mathcal{N}(\mu=0,\sigma=0.852144)$ &  $ -0.061 \pm 0.036 $  \\
fk=PR110048_TG017601_V0200 flux trend polynomial 1 & $\mathcal{N}(\mu=0,\sigma=0.313486)$ &  $ -0.03 \pm 0.13 $  \\
Log photometric scatter, $\log{\sigma_{{\rm Cheops},s}/(\rm{ppt})}$  & $\mathcal{N}(\mu=-7.578,\sigma=3) $ &  $ -7.7 \pm 2.9 $  \\
BSpline 1 , $F(\Phi)_{{\rm BS},1}$   & $\mathcal{N}(\mu=0.0,\sigma=0.0)$ &  $ 0.166^{+0.096}_{-0.093} $  \\
BSpline 2 , $F(\Phi)_{{\rm BS},2}$   & $\mathcal{N}(\mu=0.0,\sigma=0.0)$ &  $ 0.031 \pm 0.096 $  \\
BSpline 3 , $F(\Phi)_{{\rm BS},3}$   & $\mathcal{N}(\mu=0.0,\sigma=0.0)$ &  $ 0.006 \pm 0.09 $  \\
BSpline 4 , $F(\Phi)_{{\rm BS},4}$   & $\mathcal{N}(\mu=0.0,\sigma=0.0)$ &  $ 0.039^{+0.088}_{-0.084} $  \\
BSpline 5 , $F(\Phi)_{{\rm BS},5}$   & $\mathcal{N}(\mu=0.0,\sigma=0.0)$ &  $ -0.029 \pm 0.08 $  \\
BSpline 6 , $F(\Phi)_{{\rm BS},6}$   & $\mathcal{N}(\mu=0.0,\sigma=0.0)$ &  $ 0.123 \pm 0.08 $  \\
BSpline 7 , $F(\Phi)_{{\rm BS},7}$   & $\mathcal{N}(\mu=0.0,\sigma=0.0)$ &  $ -0.118 \pm 0.078 $  \\
BSpline 8 , $F(\Phi)_{{\rm BS},8}$   & $\mathcal{N}(\mu=0.0,\sigma=0.0)$ &  $ -0.006 \pm 0.076 $  \\
BSpline 9 , $F(\Phi)_{{\rm BS},9}$   & $\mathcal{N}(\mu=0.0,\sigma=0.0)$ &  $ -0.151^{+0.077}_{-0.074} $  \\
BSpline 10 , $F(\Phi)_{{\rm BS},10}$   & $\mathcal{N}(\mu=0.0,\sigma=0.0)$ &  $ -0.136 \pm 0.072 $  \\
BSpline 11 , $F(\Phi)_{{\rm BS},11}$   & $\mathcal{N}(\mu=0.0,\sigma=0.0)$ &  $ -0.012 \pm 0.071 $  \\
BSpline 12 , $F(\Phi)_{{\rm BS},12}$   & $\mathcal{N}(\mu=0.0,\sigma=0.0)$ &  $ -0.094 \pm 0.071 $  \\
BSpline 13 , $F(\Phi)_{{\rm BS},13}$   & $\mathcal{N}(\mu=0.0,\sigma=0.0)$ &  $ 0.073 \pm 0.07 $  \\
BSpline 14 , $F(\Phi)_{{\rm BS},14}$   & $\mathcal{N}(\mu=0.0,\sigma=0.0)$ &  $ 0.012 \pm 0.071 $  \\
BSpline 15 , $F(\Phi)_{{\rm BS},15}$   & $\mathcal{N}(\mu=0.0,\sigma=0.0)$ &  $ 0.108 \pm 0.071 $  \\
BSpline 16 , $F(\Phi)_{{\rm BS},16}$   & $\mathcal{N}(\mu=0.0,\sigma=0.0)$ &  $ -0.092 \pm 0.074 $  \\
BSpline 17 , $F(\Phi)_{{\rm BS},17}$   & $\mathcal{N}(\mu=0.0,\sigma=0.0)$ &  $ 0.166 \pm 0.076 $  \\
BSpline 18 , $F(\Phi)_{{\rm BS},18}$   & $\mathcal{N}(\mu=0.0,\sigma=0.0)$ &  $ -0.082 \pm 0.074 $  \\
BSpline 19 , $F(\Phi)_{{\rm BS},19}$   & $\mathcal{N}(\mu=0.0,\sigma=0.0)$ &  $ 0.016^{+0.076}_{-0.075} $  \\
BSpline 20 , $F(\Phi)_{{\rm BS},20}$   & $\mathcal{N}(\mu=0.0,\sigma=0.0)$ &  $ 0.053^{+0.075}_{-0.076} $  \\
BSpline 21 , $F(\Phi)_{{\rm BS},21}$   & $\mathcal{N}(\mu=0.0,\sigma=0.0)$ &  $ -0.074 \pm 0.077 $  \\
BSpline 22 , $F(\Phi)_{{\rm BS},22}$   & $\mathcal{N}(\mu=0.0,\sigma=0.0)$ &  $ 0.111 \pm 0.083 $  \\
BSpline 23 , $F(\Phi)_{{\rm BS},23}$   & $\mathcal{N}(\mu=0.0,\sigma=0.0)$ &  $ -0.157 \pm 0.093 $  \\
BSpline 24 , $F(\Phi)_{{\rm BS},24}$   & $\mathcal{N}(\mu=0.0,\sigma=0.0)$ &  $ 0.22 \pm 0.1 $  \\
BSpline 25 , $F(\Phi)_{{\rm BS},25}$   & $\mathcal{N}(\mu=0.0,\sigma=0.0)$ &  $ -0.21 \pm 0.11 $  \\


==> macro.tex <==
\newcommand{\TTeff}{ $ 5611.0 \pm 31.0 $ }
\newcommand{\TTeffshort}{ $ 5610.0 $ }

\newcommand{\TRs}{ $ 0.9662 \pm 0.0048 $ }
\newcommand{\TRsshort}{ $ 0.966 $ }

\newcommand{\Tg}{ $ 85.6^{+1.4}_{-3.0} $ }
\newcommand{\Tgshort}{ $ 86.0 $ }

\newcommand{\Tlogg}{ $ 4.45^{+0.016}_{-0.036} $ }
\newcommand{\Tloggshort}{ $ 4.45 $ }

\newcommand{\TKzero}{ $ 3.81 \pm 0.51 $ }
\newcommand{\TKzeroshort}{ $ 3.8 $ }

\newcommand{\TlogKzero}{ $ 1.34^{+0.12}_{-0.15} $ }
\newcommand{\TlogKzeroshort}{ $ 1.3 $ }

\newcommand{\TKone}{ $ 0.4^{+0.71}_{-0.4} $ }
\newcommand{\TKoneshort}{ $ 0.4 $ }

\newcommand{\TlogKone}{ $ -0.9^{+1.0}_{-8.7} $ }
\newcommand{\TlogKoneshort}{ $ -1.0 $ }

\newcommand{\Ttzerozero}{ $ 1767.42091 \pm 0.00059 $ }
\newcommand{\Ttzerozeroshort}{ $ 1767.4209 $ }

\newcommand{\Ttzeroone}{ $ 1779.192 \pm 0.001 $ }
\newcommand{\Ttzerooneshort}{ $ 1779.192 $ }

\newcommand{\Tperiodzero}{ $ 20.772908 \pm 2.3e-05 $ }
\newcommand{\Tperiodzeroshort}{ $ 20.77291 $ }

\newcommand{\Tperiodone}{ $ 52.56352 \pm 7e-05 $ }
\newcommand{\Tperiodoneshort}{ $ 52.56352 $ }

\newcommand{\Trvoffsetszero}{ $ -16082.61 \pm 0.58 $ }
\newcommand{\Trvoffsetszeroshort}{ $ -16082.6 $ }

\newcommand{\Trvoffsetsone}{ $ -11.38 \pm 0.35 $ }
\newcommand{\Trvoffsetsoneshort}{ $ -11.4 $ }

\newcommand{\Trvtrendzero}{ $ -5.2e-06 \pm 4e-07 $ }
\newcommand{\Trvtrendzeroshort}{ $ -5.2e-06 $ }

\newcommand{\Trvtrendone}{ $ -0.067 \pm 0.001 $ }
\newcommand{\Trvtrendoneshort}{ $ -0.067 $ }

\newcommand{\Trvtrendtwo}{ $ 0.0 \pm 5.0 $ }
\newcommand{\Trvtrendtwoshort}{ $ 0.0 $ }

\newcommand{\Tsphot}{ $ 0.5606^{+0.0068}_{-0.0064} $ }
\newcommand{\Tsphotshort}{ $ 0.561 $ }

\newcommand{\Tlogsphot}{ $ -0.579 \pm 0.012 $ }
\newcommand{\Tlogsphotshort}{ $ -0.58 $ }

\newcommand{\Tdfdsinrollanglezero}{ $ -0.013^{+0.036}_{-0.034} $ }
\newcommand{\Tdfdsinrollanglezeroshort}{ $ -0.01 $ }

\newcommand{\Tdfdcosrollanglezero}{ $ 0.064 \pm 0.026 $ }
\newcommand{\Tdfdcosrollanglezeroshort}{ $ 0.06 $ }

\newcommand{\Tdfdbgzero}{ $ 0.71 \pm 0.92 $ }
\newcommand{\Tdfdbgzeroshort}{ $ 0.7 $ }

\newcommand{\Tcheopsmeanzero}{ $ 0.423 \pm 0.027 $ }
\newcommand{\Tcheopsmeanzeroshort}{ $ 0.42 $ }

\newcommand{\Tscheops}{ $ 0.121 \pm 0.02 $ }
\newcommand{\Tscheopsshort}{ $ 0.12 $ }

\newcommand{\Tlogscheops}{ $ -2.11^{+0.15}_{-0.19} $ }
\newcommand{\Tlogscheopsshort}{ $ -2.1 $ }

\newcommand{\TMs}{ $ 1.021^{+0.043}_{-0.082} $ }
\newcommand{\TMsshort}{ $ 1.02 $ }

\newcommand{\Trorzero}{ $ 0.03708 \pm 0.00037 $ }
\newcommand{\Trorzeroshort}{ $ 0.0371 $ }

\newcommand{\Tlogrorzero}{ $ -3.295 \pm 0.01 $ }
\newcommand{\Tlogrorzeroshort}{ $ -3.29 $ }

\newcommand{\Trorone}{ $ 0.03183^{+0.00035}_{-0.00035} $ }
\newcommand{\Troroneshort}{ $ 0.0318 $ }

\newcommand{\Tlogrorone}{ $ -3.447 \pm 0.011 $ }
\newcommand{\Tlogroroneshort}{ $ -3.45 $ }

\newcommand{\Trplzero}{ $ 3.909 \pm 0.044 $ }
\newcommand{\Trplzeroshort}{ $ 3.91 $ }

\newcommand{\Trplone}{ $ 3.356 \pm 0.04 $ }
\newcommand{\Trploneshort}{ $ 3.36 $ }

\newcommand{\Tbzero}{ $ 0.13 \pm 0.12 $ }
\newcommand{\Tbzeroshort}{ $ 0.1 $ }

\newcommand{\Tbone}{ $ 0.24^{+0.089}_{-0.062} $ }
\newcommand{\Tboneshort}{ $ 0.24 $ }

\newcommand{\Tustartesszero}{ $ 0.303^{+0.061}_{-0.068} $ }
\newcommand{\Tustartesszeroshort}{ $ 0.3 $ }

\newcommand{\Tustartessone}{ $ 0.22 \pm 0.087 $ }
\newcommand{\Tustartessoneshort}{ $ 0.22 $ }

\newcommand{\Tustarcheopszero}{ $ 0.498 \pm 0.064 $ }
\newcommand{\Tustarcheopszeroshort}{ $ 0.5 $ }

\newcommand{\Tustarcheopsone}{ $ 0.205 \pm 0.081 $ }
\newcommand{\Tustarcheopsoneshort}{ $ 0.2 $ }

\newcommand{\TMpzero}{ $ 16.3 \pm 2.2 $ }
\newcommand{\TMpzeroshort}{ $ 16.0 $ }

\newcommand{\TMpone}{ $ 2.3^{+4.2}_{-2.3} $ }
\newcommand{\TMponeshort}{ $ 2.0 $ }

\newcommand{\Trhopgcmthreezero}{ $ 1.5 \pm 0.22 $ }
\newcommand{\Trhopgcmthreezeroshort}{ $ 1.5 $ }

\newcommand{\Trhopgcmthreeone}{ $ 0.34^{+0.62}_{-0.34} $ }
\newcommand{\Trhopgcmthreeoneshort}{ $ 0.3 $ }

\newcommand{\TaRszero}{ $ 32.02^{+0.45}_{-0.88} $ }
\newcommand{\TaRszeroshort}{ $ 32.0 $ }

\newcommand{\TaRsone}{ $ 59.5^{+0.8}_{-1.6} $ }
\newcommand{\TaRsoneshort}{ $ 59.0 $ }

\newcommand{\Tsmazero}{ $ 0.1437^{+0.0025}_{-0.004} $ }
\newcommand{\Tsmazeroshort}{ $ 0.144 $ }

\newcommand{\Tsmaone}{ $ 0.2668^{+0.0047}_{-0.0075} $ }
\newcommand{\Tsmaoneshort}{ $ 0.267 $ }

\newcommand{\TSinzero}{ $ 55000^{+3100}_{-1900} $ }
\newcommand{\TSinzeroshort}{ $ 55000.0 $ }

\newcommand{\TSinone}{ $ 15940^{+900}_{-560} $ }
\newcommand{\TSinoneshort}{ $ 15900.0 $ }

\newcommand{\TTsurfpzero}{ $ 663.5^{+9.2}_{-6.0} $ }
\newcommand{\TTsurfpzeroshort}{ $ 664.0 $ }

\newcommand{\TTsurfpone}{ $ 486.9^{+6.7}_{-4.4} $ }
\newcommand{\TTsurfponeshort}{ $ 487.0 $ }

\newcommand{\Ttdurzero}{ $ 0.2048^{+0.0016}_{-0.0015} $ }
\newcommand{\Ttdurzeroshort}{ $ 0.205 $ }

\newcommand{\Ttdurone}{ $ 0.2728 \pm 0.0013 $ }
\newcommand{\Ttduroneshort}{ $ 0.273 $ }

\newcommand{\TTIC}{306263608}
\newcommand{\Tra}{30.9042722461231}
\newcommand{\Tdec}{21.2808637598307}
\newcommand{\THIP}{9618}
\newcommand{\TTYC}{1213-01071-1}
\newcommand{\TGAIA}{94468978202180352}
\newcommand{\Tcontratio}{0.000620889768}
\newcommand{\TTmag}{ $ 8.5725 \pm 0.006 $ }
\newcommand{\TTmagshort}{ $ 8.572 $ }

\newcommand{\TGAIAmag}{ $ 9.02543 \pm 0.00027 $ }
\newcommand{\TGAIAmagshort}{ $ 9.0254 $ }

\newcommand{\TVmag}{ $ 9.2 \pm 0.03 $ }
\newcommand{\TVmagshort}{ $ 9.2 $ }

\newcommand{\TJmag}{ $ 7.922 \pm 0.021 $ }
\newcommand{\TJmagshort}{ $ 7.92 $ }

\newcommand{\THmag}{ $ 7.656 \pm 0.036 $ }
\newcommand{\THmagshort}{ $ 7.66 $ }

\newcommand{\TKmag}{ $ 7.559 \pm 0.021 $ }
\newcommand{\TKmagshort}{ $ 7.56 $ }

\newcommand{\Twonemag}{ $ 7.489 \pm 0.034 $ }
\newcommand{\Twonemagshort}{ $ 7.49 $ }

\newcommand{\Twtwomag}{ $ 7.563 \pm 0.021 $ }
\newcommand{\Twtwomagshort}{ $ 7.56 $ }

\newcommand{\Twthreemag}{ $ 7.547 \pm 0.018 $ }
\newcommand{\Twthreemagshort}{ $ 7.55 $ }



==> oldacknowledgements.tex <==
This work has been carried out within the framework of the National Centre of Competence in Research PlanetS supported by the Swiss National Science Foundation under grants 51NF40\_182901 and 51NF40\_205606. The authors acknowledge the financial support of the SNSF.\\ %Hugh P. Osborn
G.N. thanks for the research funding from the Ministry of Education and Science programme the "Excellence Initiative - Research University" conducted at the Centre of Excellence in Astrophysics and Astrochemistry of the Nicolaus Copernicus University in Toru\'n, Poland.\\ %Grzegorz Nowak
J.L-B. acknowledges financial support received from "la Caixa" Foundation (ID 100010434) and from the European Unions Horizon 2020 research and innovation programme under the Marie Slodowska-Curie grant agreement No 847648, with fellowship code LCF/BQ/PI20/11760023. This research has also been partly funded by the Spanish State Research Agency (AEI) Projects No. PID2019-107061GB-C61.\\ %Jorge Lillo Box
This work is partly financed by the Spanish Ministry of Economics and Competitiveness through grants PGC2018-098153-B-C31\\ %Enric Pallé
V.A acknowledges support by FCT - Funda\c{c}\~ao para a Ci\^encia e a Tecnologia (Portugal) through national funds and by FEDER through COMPETE2020 - Programa Operacional Competitividade e Internacionaliza\c{c}\~ao by these grants: UID/FIS/04434/2019; UIDB/04434/2020; UIDP/04434/2020; PTDC/FIS-AST/32113/2017 \& POCI-01-0145-FEDER-032113; PTDC/FIS-AST/28953/2017 \& POCI-01-0145-FEDER-028953.\\ %V. Adibekyan
ABr was supported by the SNSA.\\ %Alexis Brandeker
(covered by Tom Wilson's acknowledgement)\\ %Andrew Collier Cameron
DG and LMS gratefully acknowledge financial support from the \emph{Cassa di Risparmio di Torino} (CRT) foundation under Grant No. 2018.2323 ``Gaseousor rocky? Unveiling the nature of small worlds''.\\ %Davide Gandolfi
MJH, HPO and YA acknowledge the support of the Swiss National Fund under grant 200020\_172746.\\ %Matthew J. Hooton
M.L. acknowledges support of the Swiss National Science Foundation under grant number PCEFP2\_194576.\\ %Monika Lendl
AT acknowledges support from an STFC PhD studentship.\\ %Amy Tuson
This work has been carried out within the framework of the NCCR PlanetS supported by the Swiss National Science Foundation.\\ %Solène Ulmer-Moll
ACC and TGW acknowledge support from STFC consolidated grant numbers ST/R000824/1 and ST/V000861/1, and UKSA grant ST/R003203/1. \\ %Thomas G. Wilson
We acknowledge support from the Spanish Ministry of Science and Innovation and the European Regional Development Fund through grants ESP2016-80435-C2-1-R, ESP2016-80435-C2-2-R, PGC2018-098153-B-C33, PGC2018-098153-B-C31, ESP2017-87676-C5-1-R, MDM-2017-0737 Unidad de Excelencia Maria de Maeztu-Centro de Astrobiologí­a (INTA-CSIC), as well as the support of the Generalitat de Catalunya/CERCA programme. The MOC activities have been supported by the ESA contract No. 4000124370.\\ %Roi Alonso
B.S, A.A.B. \& M.V.G. acknowledge the support of Ministry of Science and Higher Education of the Russian Federation under the grant 075-15-2020-780 (N13.1902.21.0039)\\ %Alexandr A. Belinski
XB, SC, DG, MF and JL acknowledge their role as ESA-appointed CHEOPS science team members.\\ %Xavier Bonfils
This project was supported by the CNES\\ %Magali Deleuil
L.D. is an F.R.S.-FNRS Postdoctoral Researcher.\\ %Laetitia Delrez
B.-O.D. acknowledges support from the Swiss National Science Foundation (PP00P2-190080).\\ %Brice-Olivier Demory
This project has received funding from the European Research Council (ERC) under the European Union's Horizon 2020 research and innovation programme (project {\sc Four Aces}; grant agreement No 724427); DE acknowledges financial support from the Swiss National Science Foundation for project 200021\_200726.\\ %David Ehrenreich
MF gratefully acknowledge the support of the Swedish National Space Agency (DNR 65/19, 174/18).\\ %Malcolm Fridlund
M.G. is an F.R.S.-FNRS Senior Research Associate.\\ %Michaël Gillon
SH gratefully acknowledges CNES funding through the grant 837319.\\ %Sergio Hoyer
KGI is the ESA CHEOPS Project Scientist and is responsible for the ESA CHEOPS Guest Observers Programme. She does not participate in, or contribute to, the definition of the Guaranteed Time Programme of the CHEOPS mission through which observations described in this paper have been taken, nor to any aspect of target selection for the programme.\\ %Kate G. Isaak
PM acknowledges support from STFC research grant number ST/M001040/1.\\ %Pierre F. L. Maxted
This work was granted access to the HPC resources of MesoPSL financed by the Region Ile de France and the project Equip@Meso (reference ANR-10-EQPX-29-01) of the programme Investissements d'Avenir supervised by the Agence Nationale pour la Recherche\\ %Jacques Laskar
This work was also partially supported by a grant from the Simons Foundation (PI Queloz, grant number 327127).\\ %Didier Queloz
Acknowledges support from the Spanish Ministry of Science and Innovation and the European Regional Development Fund through grant PGC2018-098153-B- C33, as well as the support of the Generalitat de Catalunya/CERCA programme.\\ %Ignasi Ribas
This work was supported by FCT - Fundação para a Ciência e a Tecnologia through national funds and by FEDER through COMPETE2020 - Programa Operacional Competitividade e Internacionalizacão by these grants: UID/FIS/04434/2019, UIDB/04434/2020, UIDP/04434/2020, PTDC/FIS-AST/32113/2017 \& POCI-01-0145-FEDER- 032113, PTDC/FIS-AST/28953/2017 \& POCI-01-0145-FEDER-028953, PTDC/FIS-AST/28987/2017 \& POCI-01-0145-FEDER-028987, O.D.S.D. is supported in the form of work contract (DL 57/2016/CP1364/CT0004) funded by national funds through FCT.\\ %Olivier D. S. Demangeon
S.G.S acknowledges the support from FCT through Investigador FCT contract nr. CEECIND/00826/2018 and  POPH/FSE (EC). This  work  was  supported  by FCT - Fundac\c{c}\~ao  para  a  Ci\^encia  e  Tecnologia through national  funds and by FEDER through COMPETE2020 - Programa Operacional Competitividade e Internacionaliza\c{c}\~ao by these grants:PTDC/FIS-AST/32113/2017 \& POCI-01-0145-FEDER-032113; PTDC/FIS-AST/28953/2017 \& POCI-01-0145-FEDER-028953; PTDC/FIS-AST/28987/2017 \& POCI-01-0145-FEDER-028987.\\ %Sergio G. Sousa
GyMSz acknowledges the support of the Hungarian National Research, Development and Innovation Office (NKFIH) grant K-125015, a a PRODEX Experiment Agreement No. 4000137122, the Lend\"ulet LP2018-7/2021 grant of the Hungarian Academy of Science and the support of the city of Szombathely.\\ %Gyula M. Szabó\\ %Gyula M. Szabó
V.V.G. is a F.R.S.-FNRS Research Associate. The Belgian participation to CHEOPS has been supported by the Belgian Federal Science Policy Office (BELSPO) in the framework of the PRODEX Program, and by the University of Li\`ege through an ARC grant for Concerted Research Actions financed by the Wallonia-Brussels Federation.\\ %Valerie Van Grootel

==> oldaffiliations.tex <==

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%.    WARNING:  DO NOT EDIT YOUR AUTHOR INFO HERE.    %
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
% Author info is auto-generated from this google spreadsheet: https://docs.google.com/spreadsheets/d/1UoPGkxtxbHmJyDH8xKfOBbkoSoMXxiD9iDZ9ilVN0tE/edit?usp=sharing 
%
\textsuperscript{\hypertarget{affil_1}{1}} Physikalisches Institut, University of Bern, Gesellsschaftstrasse 6, 3012 Bern, Switzerland\\
\textsuperscript{\hypertarget{affil_2}{2}} Department of Physics and Kavli Institute for Astrophysics and Space Research, Massachusetts Institute of Technology, Cambridge, MA 02139, USA\\
\textsuperscript{\hypertarget{affil_3}{3}} Instituto de Astrofisica de Canarias, 38200 La Laguna, Tenerife, Spain\\
\textsuperscript{\hypertarget{affil_4}{4}} Departamento de Astrofisica, Universidad de La Laguna, 38206 La Laguna, Tenerife, Spain\\
\textsuperscript{\hypertarget{affil_5}{5}} Institut d'astrophysique de Paris, UMR7095 CNRS, Universit\'e Pierre \& Marie Curie, 98bis boulevard Arago, 75014 Paris, France\\
\textsuperscript{\hypertarget{affil_6}{6}} Centro de Astrobiologi\'ia (CAB,CSIC-INTA), Dep. de Astrof\'isica, ESAC campus, 28692, Villanueva de la Ca\~nada, Madrid, Spain\\
\textsuperscript{\hypertarget{affil_7}{7}} Deptartamento de Astrofisica, Universidad de La Laguna (ULL), E-38206 La Laguna, Tenerife, Spain\\
\textsuperscript{\hypertarget{affil_8}{8}} Observatoire Astronomique de l'Université de Genève, Chemin Pegasi 51, CH-1290 Versoix, Switzerland\\
\textsuperscript{\hypertarget{affil_9}{9}} Department of Astronomy, Stockholm University, AlbaNova University Center, 10691 Stockholm, Sweden\\
\textsuperscript{\hypertarget{affil_10}{10}} Aix Marseille Univ, CNRS, CNES, LAM, 38 rue Frédéric Joliot-Curie, 13388 Marseille, France; Division Technique INSU, CS20330, 83507 La Seyne sur Mer cedex, France\\
\textsuperscript{\hypertarget{affil_11}{11}} Instituto de Astrof\'isica e Ci\^encias do Espa\c{c}o, Universidade do Porto, CAUP, Rua das Estrelas, 4150-762 Porto, Portugal\\
\textsuperscript{\hypertarget{affil_12}{12}} Center for Astrophysics \textbar Harvard \& Smithsonian, 60 Garden Street, Cambridge, MA 02138, USA\\
\textsuperscript{\hypertarget{affil_13}{13}} NASA Exoplanet Science Institute - Caltech/IPAC, Pasadena, CA 91125 USA\\
\textsuperscript{\hypertarget{affil_14}{14}} Centre for Exoplanet Science, SUPA School of Physics and Astronomy, University of St Andrews, North Haugh, St Andrews KY16 9SS, UK\\
\textsuperscript{\hypertarget{affil_15}{15}} Dipartimento di Fisica, Universita degli Studi di Torino, via Pietro Giuria 1, I-10125, Torino, Italy\\
\textsuperscript{\hypertarget{affil_16}{16}} Astrophysics Group, Cavendish Laboratory, University of Cambridge, J.J. Thomson Avenue, Cambridge CB3 0HE, UK\\
\textsuperscript{\hypertarget{affil_17}{17}} Observatoire Astronomique de l'Université de Genève, Chemin Pegasi 51, Versoix, Switzerland\\
\textsuperscript{\hypertarget{affil_18}{18}} Department of Physics, Engineering and Astronomy, Stephen F. Austin State University, 1936 North St, Nacogdoches, TX 75962, USA\\
\textsuperscript{\hypertarget{affil_19}{19}} Institut de Ciencies de l'Espai (ICE, CSIC), Campus UAB, Can Magrans s/n, 08193 Bellaterra, Spain\\
\textsuperscript{\hypertarget{affil_20}{20}} Institut d'Estudis Espacials de Catalunya (IEEC), 08034 Barcelona, Spain\\
\textsuperscript{\hypertarget{affil_21}{21}} Observatoire de Haute-Provence, CNRS, Universit\'e d'Aix-Marseille, 04870 Saint-Michel-l'Observatoire, France\\
\textsuperscript{\hypertarget{affil_22}{22}} ESTEC, European Space Agency, 2201AZ, Noordwijk, NL\\
\textsuperscript{\hypertarget{affil_23}{23}} Depto. de Astrofisica, Centro de Astrobiologia (CSIC-INTA), ESAC campus, 28692 Villanueva de la Cañada (Madrid), Spain\\
\textsuperscript{\hypertarget{affil_24}{24}} Space Research Institute, Austrian Academy of Sciences, Schmiedlstrasse 6, A-8042 Graz, Austria\\
\textsuperscript{\hypertarget{affil_25}{25}} Sternberg Astronomical Institute Lomonosov Moscow State University, Universitetskii prospekt, 13, Moscow, 119992, Russia\\
\textsuperscript{\hypertarget{affil_26}{26}} Center for Space and Habitability, University of Bern, Gesellschaftsstrasse 6, 3012, Bern, Switzerland\\
\textsuperscript{\hypertarget{affil_27}{27}} Max Planck Institute for Extraterrestrial Physics\\
\textsuperscript{\hypertarget{affil_28}{28}} INAF - Osservatorio Astronomico di Padova\\
\textsuperscript{\hypertarget{affil_29}{29}} Laboratoire d'Astrophysique de Marseille, Universit\'e de Provence, UMR6110 CNRS, 38 rue F. Joliot Curie, 13388 Marseille cedex 13, France\\
\textsuperscript{\hypertarget{affil_30}{30}} Université Grenoble Alpes, CNRS, IPAG, 38000 Grenoble, France\\
\textsuperscript{\hypertarget{affil_31}{31}} 1DTU Space, National Space Institute, Technical University of Denmark, Elektrovej 328, DK-2800 Kgs. Lyngby, Denmark\\
\textsuperscript{\hypertarget{affil_32}{32}} Admatis, 5. Kandó Kálmán Street, 3534 Miskolc, Hungary\\
\textsuperscript{\hypertarget{affil_33}{33}} Instituto de Astrofisica e Ciencias do Espaco, Universidade do Porto, CAUP, Rua das Estrelas, 4150-762 Porto, Portugal\\
\textsuperscript{\hypertarget{affil_34}{34}} Departamento de Fisica e Astronomia, Faculdade de Ciencias, Universidade do Porto, Rua do Campo Alegre, 4169-007 Porto, Portugal\\
\textsuperscript{\hypertarget{affil_35}{35}} Institute of Planetary Research, German Aerospace Center (DLR), Rutherfordstrasse 2, 12489 Berlin, Germany\\
\textsuperscript{\hypertarget{affil_36}{36}} Université de Paris, Institut de physique du globe de Paris, CNRS, F-75005 Paris, France\\
\textsuperscript{\hypertarget{affil_37}{37}} Centre for Mathematical Sciences, Lund University, Box 118, 22100 Lund, Sweden\\
\textsuperscript{\hypertarget{affil_38}{38}} Aix Marseille Univ, CNRS, CNES, LAM, 38 rue Frédéric Joliot-Curie, 13388 Marseille, France\\
\textsuperscript{\hypertarget{affil_39}{39}} Universit\'e Grenoble Alpes, CNRS, IPAG, 38000 Grenoble, France\\
\textsuperscript{\hypertarget{affil_40}{40}} Astrobiology Research Unit, Université de Liège, Allée du 6 Août 19C, B-4000 Liège, Belgium\\
\textsuperscript{\hypertarget{affil_41}{41}} Space sciences, Technologies and Astrophysics Research (STAR) Institute, Universit\'e de Li\`ege, 19C All\'ee du 6 Ao\^ut, B-4000 Li\`ege, Belgium\\
\textsuperscript{\hypertarget{affil_42}{42}} Center for Space and Habitability, Gesellsschaftstrasse 6, 3012 Bern, Switzerland\\
\textsuperscript{\hypertarget{affil_43}{43}} Lunar and Planetary Laboratory, The University of Arizona, Tucson, AZ 85721, USA\\
\textsuperscript{\hypertarget{affil_44}{44}} Leiden Observatory, University of Leiden, PO Box 9513, 2300 RA Leiden, The Netherlands\\
\textsuperscript{\hypertarget{affil_45}{45}} Department of Space, Earth and Environment, Chalmers University of Technology, Onsala Space Observatory, 43992 Onsala, Sweden\\
\textsuperscript{\hypertarget{affil_46}{46}} Department of Astronomy and Astrophysics, University of California, Santa Cruz, CA 95064, USA\\
\textsuperscript{\hypertarget{affil_47}{47}} Department of Astrophysics, University of Vienna, Tuerkenschanzstrasse 17, 1180 Vienna, Austria\\
\textsuperscript{\hypertarget{affil_48}{48}} NASA Ames Research Center, Moffett Field, CA 94035, USA\\
\textsuperscript{\hypertarget{affil_49}{49}} Science and Operations Department - Science Division (SCI-SC), Directorate of Science, European Space Agency (ESA), European Space Research and Technology Centre (ESTEC), Keplerlaan 1, 2201-AZ Noordwijk, The Netherlands\\
\textsuperscript{\hypertarget{affil_50}{50}} Konkoly Observatory, Research Centre for Astronomy and Earth Sciences, 1121 Budapest, Konkoly Thege Miklós út 15-17, Hungary\\
\textsuperscript{\hypertarget{affil_51}{51}} ELTE E\”otv\”os Lor\'and University, Institute of Physics, P\'azm\'any P\'eter s\'et\'any 1/A, 1117 Budapest, Hungary\\
\textsuperscript{\hypertarget{affil_52}{52}} Rheinisches Institut für Umweltforschung an der Universität zu Köln, D-50931 Köln, Germany.\\
\textsuperscript{\hypertarget{affil_53}{53}} Department of Space, Earth and Environment, Astronomy and Plasma Physics, Chalmers University of Technology, 412 96 Gothenburg, Sweden.\\
\textsuperscript{\hypertarget{affil_54}{54}} Astrophysics Group, Keele University, Staffordshire, ST5 5BG, United Kingdom\\
\textsuperscript{\hypertarget{affil_55}{55}} IMCCE, UMR8028 CNRS, Observatoire de Paris, PSL Univ., Sorbonne Univ., 77 av. Denfert-Rochereau, 75014 Paris, France\\
\textsuperscript{\hypertarget{affil_56}{56}} Institut d'astrophysique de Paris, UMR7095 CNRS, Université Pierre \& Marie Curie, 98bis blvd. Arago, 75014 Paris, France\\
\textsuperscript{\hypertarget{affil_57}{57}} Department of Astronomy & Astrophysics, University of Chicago, Chicago, IL 60637, USA.\\
\textsuperscript{\hypertarget{affil_58}{58}} INAF, Osservatorio Astronomico di Padova, Vicolo dell'Osservatorio 5, 35122 Padova, Italy\\
\textsuperscript{\hypertarget{affil_59}{59}} Laborat\'{o}rio Nacional de Astrof\'{i}sica, Rua Estados Unidos 154, 37504-364, Itajub\'{a} - MG, Brazil\\
\textsuperscript{\hypertarget{affil_60}{60}} Space Telescope Science Institute, 3700 San Martin Drive, Baltimore, MD, 21218, USA\\
\textsuperscript{\hypertarget{affil_61}{61}} Google, Cambridge, MA, USA\\
\textsuperscript{\hypertarget{affil_62}{62}} Universit\'e de Toulouse, CNRS, IRAP, 14 avenue Belin, 31400 Toulouse, France\\
\textsuperscript{\hypertarget{affil_63}{63}} Department of Physics \& Astronomy, Swarthmore College, Swarthmore PA 19081, USA\\
\textsuperscript{\hypertarget{affil_64}{64}} INAF, Osservatorio Astrofisico di Catania, Via S. Sofia 78, 95123 Catania, Italy\\
\textsuperscript{\hypertarget{affil_65}{65}} Dipartimento di Fisica e Astronomia "Galileo Galilei", Universita degli Studi di Padova, Vicolo dell'Osservatorio 3, 35122 Padova, Italy\\
\textsuperscript{\hypertarget{affil_66}{66}} Department of Physics, University of Warwick, Gibbet Hill Road, Coventry CV4 7AL, United Kingdom\\
\textsuperscript{\hypertarget{affil_67}{67}} Cavendish Laboratory, JJ Thomson Avenue, Cambridge CB3 0HE, UK\\
\textsuperscript{\hypertarget{affil_68}{68}} Center for Astronomy and Astrophysics, Technical University Berlin, Hardenberstrasse 36, 10623 Berlin, Germany\\
\textsuperscript{\hypertarget{affil_69}{69}} ELTE E\”otv\”os Lor\'and University, Gothard Astrophysical Observatory, 9700 Szombathely, Szent Imre h. u. 112, Hungary\\
\textsuperscript{\hypertarget{affil_70}{70}} MTA-ELTE Exoplanet Research Group, 9700 Szombathely, Szent Imre h. u. 112, Hungary\\
\textsuperscript{\hypertarget{affil_71}{71}} German Aerospace Center (DLR), Institute of Optical Sensor Systems, Rutherfordstraße 2, 12489 Berlin\\
\textsuperscript{\hypertarget{affil_72}{72}} Institute of Astronomy, University of Cambridge, Madingley Road, Cambridge, CB3 0HA, United Kingdom\\
\textsuperscript{\hypertarget{affil_73}{73}} Department of Astrophysical Sciences, Princeton University, 4 Ivy Lane, Princeton, NJ 08544, USA\\


==> oldauthorlist.tex <==
\author{H.~P.~Osborn\inst{1}\fnmsep\inst{2}\textsuperscript{,\orcidicon{0000-0002-4047-4724}}\thanks{E-mail:hugh.osborn@unibe.ch} , % hugh.osborn@space.unibe.ch First author
\textbf{Author list TBD \& pending Cheops GTO approval}, 
J.~A.~Egger\inst{1} , % jo-ann.egger@unibe.ch Interior structure modelling
G.~Hébrard\inst{3} , % hebrard@iap.fr Sophie RVs
T.~Masseron\inst{4}\fnmsep\inst{5} , % thomas.masseron@iac.es HARPS-N RVs and stellar side
G.~Nowak\inst{4}\fnmsep\inst{5} , % gnowak@iac.es HARPS-N RVs
V.~Adibekyan\inst{6}\orcidicon{0000-0002-0601-6199} , % Vardan.Adibekyan@astro.up.pt Stellar abundances and ages
A.~Bieryla\inst{7}\orcidicon{0000-0001-6637-5401} , % abieryla@cfa.harvard.edu TRES stellar parameters
A.~Brandeker\inst{8}\orcidicon{0000-0002-7201-7536} , % alexis@astro.su.se Cheops GTO team
L.~A.~Buchhave\inst{9}\orcidicon{0000-0003-1605-5666} , % buchhave@space.dtu.dk FIES spectra
D.~R.~Ciardi\inst{10}\orcidicon{0000-0002-5741-3047} , % ciardi@ipac.caltech.edu Palomar and Keck NIR AO data
A.~Collier~Cameron\inst{11}\orcidicon{0000-0002-8863-7828} , % acc4@st-andrews.ac.uk Cheops GTO team
K.~A.~Collins\inst{12}\orcidicon{0000-0001-6588-9574} , % karen.collins@cfa.harvard.edu SG1 coordination and data analysis
D.~Gandolfi\inst{13}\orcidicon{0000-0001-8627-9628} , % davide.gandolfi@unito.it Advisor to Cheops duotransits team & Explore Program manager
M.~Lendl\inst{14}\orcidicon{0000-0001-9699-1459} , % monika.lendl@oeaw.ac.at Advisor to Cheops duotransits team
E.~Matthews\inst{14}\orcidicon{0000-0003-0593-1560} , % elisabeth.matthews@unige.ch Companion discussions
E.~Pallé\inst{4}\fnmsep\inst{15}\orcidicon{0000-0003-0987-1593} , % epalle@iac.es Cheops GTO team
A.~Tuson\inst{16}\orcidicon{0000-0002-2830-9064} , % alt59@cam.ac.uk Key member of Cheops duotransits team
S.~Ulmer-Moll\inst{14}\orcidicon{0000-0003-2417-7006} , % solene.ulmer-moll@unige.ch Key member of Cheops duotransits team
A.~Vanderburg\inst{2} , % andrew.m.vanderburg@gmail.com Quaternion Detrending
T.~G.~Wilson\inst{11}\orcidicon{0000-0001-8749-1962} , % tgw1@st-andrews.ac.uk Stellar parameters
C.~Ziegler\inst{17} , % carlziegler@gmail.com LCO + SOAR
Robert~F.~Goeke\inst{2} , % goeke@space.mit.edu POC nomination
Y.~Alibert\inst{1}\orcidicon{0000-0002-4644-8818} , % yann.alibert@unibe.ch Cheops GTO team
R.~Alonso\inst{4}\fnmsep\inst{5}\orcidicon{0000-0001-8462-8126} , % ras@iac.es Cheops GTO team
G.~Anglada\inst{18}\fnmsep\inst{19} , % anglada@ice.csic.es Cheops GTO team
L.~Arnold\inst{20} , % Luc.Arnold@osupytheas.fr Sophie
D.~Barrado~y~Navascues\inst{21} , % barrado@cab.inta-csic.es Cheops GTO team
W.~Baumjohann\inst{22}\orcidicon{0000-0001-6271-0110} , % baumjohann@oeaw.ac.at Cheops GTO team
T.~Beck\inst{1} , % thomas.beck@csh.unibe.ch Cheops GTO team
A.~A.~Belinski\inst{23}\orcidicon{0000-0003-3469-0989} , % aleks.sai@gmail.com SAI-2.5m speckle data
W.~Benz\inst{1}\fnmsep\inst{24} , % willy.benz@unibe.ch Cheops GTO team
A.~Bieryla\inst{7} , % abieryla@cfa.harvard.edu TRES spectra/stellar parameters
I.~Boisse\inst{25} , % isabelle.boisse@lam.fr Sophie
X.~Bonfils\inst{26} , % xavier.bonfils@obs.ujf-grenoble.fr Cheops GTO team
C.~Broeg\inst{1}\fnmsep\inst{24}\orcidicon{0000-0001-5132-2614} , % christopher.broeg@unibe.ch Cheops GTO team
T.~Bárczy\inst{27} , % tamas.barczy@admatis.com Cheops GTO team
S.C.C.~Barros\inst{28}\fnmsep\inst{29}\orcidicon{0000-0003-2434-3625} , % susana.barros@astro.up.pt Cheops GTO team
J.~Cabrera\inst{30}\orcidicon{0000-0001-6653-5487} , % juan.cabrera@dlr.de Cheops GTO team
S.~Charnoz\inst{31} , % charnoz@ipgp.fr Cheops GTO team
J.~Christiansen\inst{10} , % christia@ipac.caltech.edu TSO nomination
P.~Cortes\inst{25} , % pia.cortes@lam.fr Sophie
S.~Csizmadia\inst{30} , % szilard.csizmadia@dlr.de Cheops GTO team
S.~Dalal\inst{3} , % shweta.dalal@iap.fr Sophie
M.~B.~Davies\inst{32}\orcidicon{0000-0001-6080-1190} , % melvyn_b.davies@math.lu.se Cheops GTO team
M.~Deleuil\inst{33} , % magali.deleuil@lam.fr Cheops GTO team
X.~Delfosse\inst{34} , % xavier.delfosse@univ-grenoble-alpes.fr Sophie
L.~Delrez\inst{35}\fnmsep\inst{36} , % ldelrez@uliege.be Cheops GTO team
B.-O.~Demory\inst{37} , % brice.demory@csh.unibe.ch Cheops GTO team
D.~Ehrenreich\inst{14} , % david.ehrenreich@unige.ch Cheops GTO team
A.~Erikson\inst{30} , % Anders.Erikson@dlr.de Cheops GTO team
R.~B.~Fernandes\inst{38}\orcidicon{0000-0002-3853-7327} , % rachelfernandes@email.arizona.edu Palomar NIR AO data
A.~Fortier\inst{1}\fnmsep\inst{24}\orcidicon{0000-0001-8450-3374} , % andrea.fortier@unibe.ch Cheops GTO team
T.~Forveille\inst{34} , % thierry.forveille@univ-grenoble-alpes.fr Sophie
L.~Fossati\inst{22} , % Luca.Fossati@oeaw.ac.at Cheops GTO team
M.~Fridlund\inst{39}\fnmsep\inst{40} , % fridlund@strw.leidenuniv.nl Cheops GTO team
E.~Furlan\inst{10} , % furlan@ipac.caltech.edu Gemini NIR AO data
M.~Gillon\inst{35} , % michael.gillon@ulg.ac.be Cheops GTO team
M.~V.~Goliguzova\inst{23}\orcidicon{0000-0003-2228-7914} , % margo1000i1@mail.ru SAI-2.5m speckle data
E.~J.~Gonzales\inst{41}\orcidicon{0000-0002-9329-2190} , % erjagonz@ucsc.edu Keck NIR AO data
M.~Güdel\inst{42} , % manuel.guedel@univie.ac.at Cheops GTO team
N.~Heidari\inst{25} , % neda.heidari@lam.fr Sophie
S.~Howell\inst{43} , % steve.b.howell@nasa.gov Gemini
S.~Hoyer\inst{33} , % sergio.hoyer@lam.fr Cheops GTO team
K.~G.~Isaak\inst{44} , % kisaak@cosmos.esa.int Cheops GTO team
J.~M.~Jenkins\inst{45}\orcidicon{0000-0002-4715-9460} , % jon.jenkins@nasa.gov TESS architects
F.~Kiefer\inst{3} , % kiefer@iap.fr Sophie
L.~Kiss\inst{46}\fnmsep\inst{47} , % kiss@konkoly.hu Cheops GTO team
P.~F.~L.~Maxted\inst{48} , % p.maxted@keele.ac.uk Cheops GTO team
J.~Laskar\inst{49} , % laskar@imcce.fr Cheops GTO team
D.~W.~Latham\inst{7}\orcidicon{0000-0001-9911-7388} , % dlatham@cfa.harvard.edu TESS architects
A.~Lecavelier~des~Etangs\inst{50} , % lecaveli@iap.fr Cheops GTO team
C.~Lovis\inst{14} , % christophe.lovis@unige.ch Cheops GTO team
M.~B.~Lund\inst{10}\orcidicon{0000-0002-4236-9020} , % mlund@ipac.caltech.edu Palomar NIR AO data
D.~Magrin\inst{51} , % demetrio.magrin@inaf.it Cheops GTO team
J.~Manuel~Almenara\inst{34} , % jose-manuel.almenara-villa@univ-grenoble-alpes.fr Sophie
E.~Martioli\inst{3}\fnmsep\inst{52} , % martioli@iap.fr Sophie
J.~V.~Medina\inst{53} , % jmedina@stsci.edu POC nomination
D.~Moldovan\inst{54} , % mdan@google.com POC nomination
C.~Moutou\inst{55} , % claire.moutou@irap.omp.eu Sophie
V.~Nascimbeni\inst{51} , % valerio.nascimbeni@inaf.it Cheops GTO team
G.~Olofsson\inst{8} , % olofsson@astro.su.se Cheops GTO team
R.~Ottensamer\inst{42} , % roland.ottensamer@univie.ac.at Cheops GTO team
I.~Pagano\inst{56} , % isabella.pagano@inaf.it Cheops GTO team
G.~Peter\inst{30} , % gisbert.peter@dlr.de Cheops GTO team
G.~Piotto\inst{57}\fnmsep\inst{51} , % giampaolo.piotto@unipd.it Cheops GTO team
D.~Pollacco\inst{58} , % d.pollacco@warwick.ac.uk Cheops GTO team
D.~Queloz\inst{14}\fnmsep\inst{59} , % didier.queloz@unige.ch Cheops GTO team
R.~Ragazzoni\inst{51}\fnmsep\inst{57} , % roberto.ragazzoni@inaf.it Cheops GTO team
N.~Rando\inst{60} , % nicola.rando@esa.int Cheops GTO team
H.~Rauer\inst{30}\fnmsep\inst{61} , % Heike.Rauer@dlr.de Cheops GTO team
I.~Ribas\inst{18}\fnmsep\inst{19} , % iribas@ice.cat Cheops GTO team
G.~Ricker\inst{2}\orcidicon{0000-0003-2058-6662} , % grr@space.mit.edu TESS architects
O.~D.~S.~Demangeon\inst{28}\fnmsep\inst{29}\orcidicon{0000-0001-7918-0355} , % olivier.demangeon@astro.up.pt Cheops GTO team
A.~M.~S.~Smith\inst{30}\orcidicon{0000-0002-2386-4341} , % alexis.smith@dlr.de Cheops GTO team
N.~Santos\inst{28}\fnmsep\inst{29} , % nuno.santos@astro.up.pt Cheops GTO team
G.~Scandariato\inst{56}\orcidicon{0000-0003-2029-0626} , % gaetano.scandariato@inaf.it Cheops GTO team
S.~Seager\inst{2}\orcidicon{0000-0002-6892-6948} , % seager@mit.edu TESS architects
A.~E.~Simon\inst{1}\orcidicon{0000-0001-9773-2600} , % attila.simon@unibe.ch Cheops GTO team
S.~G.~Sousa\inst{28}\orcidicon{0000-0001-9047-2965} , % sergio.sousa@astro.up.pt Stellar parameters
M.~Steller\inst{22} , % Manfred.Steller@oeaw.ac.at Cheops GTO team
G.~M.~Szabó\inst{62}\fnmsep\inst{63} , % szgy@konkoly.hu; szgy@gothard.hu Cheops GTO team
D.~Ségransan\inst{14} , % damien.segransan@unige.ch Cheops GTO team
N.~Thomas\inst{1} , % nicolas.thomas@unibe.ch Cheops GTO team
S.~Udry\inst{14}\orcidicon{0000-0001-7576-6236} , % stephane.udry@unige.ch Cheops GTO team
B.~Ulmer\inst{30} , % bernd.ulmer@dlr.de Gisbert (Cheops MA) nomination
V.~Van~Grootel\inst{64}\orcidicon{0000-0003-2144-4316} , % valerie.vangrootel@uliege.be Stellar parameters
R.~Vanderspek\inst{2}\orcidicon{0000-0001-6763-6562} , % roland@space.mit.edu TESS architects
N.~Walton\inst{65} , % naw@ast.cam.ac.uk Cheops GTO team
J.~N.~Winn\inst{66}\orcidicon{0000-0002-4265-047X} , % jnwinn@princeton.edu TESS architects
E.~L.\~N.\~Jensen\inst{67}\orcidicon{0000-0002-4625-7333} % ejensen1@swarthmore.edu LCO observations
}\\
\vspace{0.4cm}
\parbox{\textwidth}{
The authors' affiliations are shown in Appendix \ref{sec:affiliations}.}
}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%.    WARNING:  DO NOT EDIT YOUR AUTHOR INFO HERE.    %
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
% Author info is auto-generated from this google spreadsheet: https://docs.google.com/spreadsheets/d/1UoPGkxtxbHmJyDH8xKfOBbkoSoMXxiD9iDZ9ilVN0tE/edit?usp=sharing 
%
\textsuperscript{\hypertarget{affil_1}{1}} Physikalisches Institut, University of Bern, Gesellsschaftstrasse 6, 3012 Bern, Switzerland\\
\textsuperscript{\hypertarget{affil_2}{2}} Department of Physics and Kavli Institute for Astrophysics and Space Research, Massachusetts Institute of Technology, Cambridge, MA 02139, USA\\
\textsuperscript{\hypertarget{affil_3}{3}} Institut d'astrophysique de Paris, UMR7095 CNRS, Universit\'e Pierre \& Marie Curie, 98bis boulevard Arago, 75014 Paris, France\\
\textsuperscript{\hypertarget{affil_4}{4}} Instituto de Astrofisica de Canarias, 38200 La Laguna, Tenerife, Spain\\
\textsuperscript{\hypertarget{affil_5}{5}} Departamento de Astrofisica, Universidad de La Laguna, 38206 La Laguna, Tenerife, Spain\\
\textsuperscript{\hypertarget{affil_6}{6}} Instituto de Astrof\'isica e Ci\^encias do Espa\c{c}o, Universidade do Porto, CAUP, Rua das Estrelas, 4150-762 Porto, Portugal\\
\textsuperscript{\hypertarget{affil_7}{7}} Center for Astrophysics | Harvard & Smithsonian, 60 Garden St, Cambridge, MA, 02138, USA\\
\textsuperscript{\hypertarget{affil_8}{8}} Department of Astronomy, Stockholm University, AlbaNova University Center, 10691 Stockholm, Sweden\\
\textsuperscript{\hypertarget{affil_9}{9}} 1DTU Space, National Space Institute, Technical University of Denmark, Elektrovej 328, DK-2800 Kgs. Lyngby, Denmark\\
\textsuperscript{\hypertarget{affil_10}{10}} NASA Exoplanet Science Institute - Caltech/IPAC, Pasadena, CA 91125 USA\\
\textsuperscript{\hypertarget{affil_11}{11}} Centre for Exoplanet Science, SUPA School of Physics and Astronomy, University of St Andrews, North Haugh, St Andrews KY16 9SS, UK\\
\textsuperscript{\hypertarget{affil_12}{12}} Center for Astrophysics \textbar \ Harvard \& Smithsonian, 60 Garden Street, Cambridge, MA 02138, USA\\
\textsuperscript{\hypertarget{affil_13}{13}} Dipartimento di Fisica, Universita degli Studi di Torino, via Pietro Giuria 1, I-10125, Torino, Italy\\
\textsuperscript{\hypertarget{affil_14}{14}} Observatoire Astronomique de l'Université de Genève, Chemin Pegasi 51, Versoix, Switzerland\\
\textsuperscript{\hypertarget{affil_15}{15}} Deptartamento de Astrofisica, Universidad de La Laguna (ULL), E-38206 La Laguna, Tenerife, Spain\\
\textsuperscript{\hypertarget{affil_16}{16}} Astrophysics Group, Cavendish Laboratory, University of Cambridge, J.J. Thomson Avenue, Cambridge CB3 0HE, UK\\
\textsuperscript{\hypertarget{affil_17}{17}} Department of Physics, Engineering and Astronomy, Stephen F. Austin State University, 1936 North St, Nacogdoches, TX 75962, USA\\
\textsuperscript{\hypertarget{affil_18}{18}} Institut de Ciencies de l'Espai (ICE, CSIC), Campus UAB, Can Magrans s/n, 08193 Bellaterra, Spain\\
\textsuperscript{\hypertarget{affil_19}{19}} Institut d'Estudis Espacials de Catalunya (IEEC), 08034 Barcelona, Spain\\
\textsuperscript{\hypertarget{affil_20}{20}} Observatoire de Haute-Provence, CNRS, Universit\'e d'Aix-Marseille, 04870 Saint-Michel-l'Observatoire, France\\
\textsuperscript{\hypertarget{affil_21}{21}} Depto. de Astrofisica, Centro de Astrobiologia (CSIC-INTA), ESAC campus, 28692 Villanueva de la Cañada (Madrid), Spain\\
\textsuperscript{\hypertarget{affil_22}{22}} Space Research Institute, Austrian Academy of Sciences, Schmiedlstrasse 6, A-8042 Graz, Austria\\
\textsuperscript{\hypertarget{affil_23}{23}} Sternberg Astronomical Institute Lomonosov Moscow State University, Universitetskii prospekt, 13, Moscow, 119992, Russia\\
\textsuperscript{\hypertarget{affil_24}{24}} Center for Space and Habitability, University of Bern, Gesellschaftsstrasse 6, 3012, Bern, Switzerland\\
\textsuperscript{\hypertarget{affil_25}{25}} Laboratoire d'Astrophysique de Marseille, Universit\'e de Provence, UMR6110 CNRS, 38 rue F. Joliot Curie, 13388 Marseille cedex 13, France\\
\textsuperscript{\hypertarget{affil_26}{26}} Université Grenoble Alpes, CNRS, IPAG, 38000 Grenoble, France\\
\textsuperscript{\hypertarget{affil_27}{27}} Admatis, 5. Kandó Kálmán Street, 3534 Miskolc, Hungary\\
\textsuperscript{\hypertarget{affil_28}{28}} Instituto de Astrofisica e Ciencias do Espaco, Universidade do Porto, CAUP, Rua das Estrelas, 4150-762 Porto, Portugal\\
\textsuperscript{\hypertarget{affil_29}{29}} Departamento de Fisica e Astronomia, Faculdade de Ciencias, Universidade do Porto, Rua do Campo Alegre, 4169-007 Porto, Portugal\\
\textsuperscript{\hypertarget{affil_30}{30}} Institute of Planetary Research, German Aerospace Center (DLR), Rutherfordstrasse 2, 12489 Berlin, Germany\\
\textsuperscript{\hypertarget{affil_31}{31}} Université de Paris, Institut de physique du globe de Paris, CNRS, F-75005 Paris, France\\
\textsuperscript{\hypertarget{affil_32}{32}} Centre for Mathematical Sciences, Lund University, Box 118, 22100 Lund, Sweden\\
\textsuperscript{\hypertarget{affil_33}{33}} Aix Marseille Univ, CNRS, CNES, LAM, 38 rue Frédéric Joliot-Curie, 13388 Marseille, France\\
\textsuperscript{\hypertarget{affil_34}{34}} Universit\'e Grenoble Alpes, CNRS, IPAG, 38000 Grenoble, France\\
\textsuperscript{\hypertarget{affil_35}{35}} Astrobiology Research Unit, Université de Liège, Allée du 6 Août 19C, B-4000 Liège, Belgium\\
\textsuperscript{\hypertarget{affil_36}{36}} Space sciences, Technologies and Astrophysics Research (STAR) Institute, Université de Liège, Allée du 6 Août 19C, 4000 Liège, Belgium\\
\textsuperscript{\hypertarget{affil_37}{37}} Center for Space and Habitability, Gesellsschaftstrasse 6, 3012 Bern, Switzerland\\
\textsuperscript{\hypertarget{affil_38}{38}} Lunar and Planetary Laboratory, The University of Arizona, Tucson, AZ 85721, USA\\
\textsuperscript{\hypertarget{affil_39}{39}} Leiden Observatory, University of Leiden, PO Box 9513, 2300 RA Leiden, The Netherlands\\
\textsuperscript{\hypertarget{affil_40}{40}} Department of Space, Earth and Environment, Chalmers University of Technology, Onsala Space Observatory, 43992 Onsala, Sweden\\
\textsuperscript{\hypertarget{affil_41}{41}} Department of Astronomy and Astrophysics, University of California, Santa Cruz, CA 95064, USA\\
\textsuperscript{\hypertarget{affil_42}{42}} Department of Astrophysics, University of Vienna, Tuerkenschanzstrasse 17, 1180 Vienna, Austria\\
\textsuperscript{\hypertarget{affil_43}{43}} NASA Ames Research Center, Moffett Field, CA 94035, USA\\
\textsuperscript{\hypertarget{affil_44}{44}} Science and Operations Department - Science Division (SCI-SC), Directorate of Science, European Space Agency (ESA), European Space Research and Technology Centre (ESTEC), Keplerlaan 1, 2201-AZ Noordwijk, The Netherlands\\
\textsuperscript{\hypertarget{affil_45}{45}} NASA Ames Research Center,Moffett Field, CA 94035, USA\\
\textsuperscript{\hypertarget{affil_46}{46}} Konkoly Observatory, Research Centre for Astronomy and Earth Sciences, 1121 Budapest, Konkoly Thege Miklós út 15-17, Hungary\\
\textsuperscript{\hypertarget{affil_47}{47}} ELTE E\”otv\”os Lor\’and University, Institute of Physics, P\’azm\’any P\’eter s\’et\’any 1/A, 1117 Budapest, Hungary\\
\textsuperscript{\hypertarget{affil_48}{48}} Astrophysics Group, Keele University, Staffordshire, ST5 5BG, United Kingdom\\
\textsuperscript{\hypertarget{affil_49}{49}} IMCCE, UMR8028 CNRS, Observatoire de Paris, PSL Univ., Sorbonne Univ., 77 av. Denfert-Rochereau, 75014 Paris, France\\
\textsuperscript{\hypertarget{affil_50}{50}} Institut d'astrophysique de Paris, UMR7095 CNRS, Université Pierre \& Marie Curie, 98bis blvd. Arago, 75014 Paris, France\\
\textsuperscript{\hypertarget{affil_51}{51}} INAF, Osservatorio Astronomico di Padova, Vicolo dell'Osservatorio 5, 35122 Padova, Italy\\
\textsuperscript{\hypertarget{affil_52}{52}} Laborat\'{o}rio Nacional de Astrof\'{i}sica, Rua Estados Unidos 154, 37504-364, Itajub\'{a} - MG, Brazil\\
\textsuperscript{\hypertarget{affil_53}{53}} Space Telescope Science Institute, 3700 San Martin Drive, Baltimore, MD, 21218, USA\\
\textsuperscript{\hypertarget{affil_54}{54}} Google, Cambridge, MA, USA\\
\textsuperscript{\hypertarget{affil_55}{55}} Universit\'e de Toulouse, CNRS, IRAP, 14 avenue Belin, 31400 Toulouse, France\\
\textsuperscript{\hypertarget{affil_56}{56}} INAF, Osservatorio Astrofisico di Catania, Via S. Sofia 78, 95123 Catania, Italy\\
\textsuperscript{\hypertarget{affil_57}{57}} Dipartimento di Fisica e Astronomia "Galileo Galilei", Universita degli Studi di Padova, Vicolo dell'Osservatorio 3, 35122 Padova, Italy\\
\textsuperscript{\hypertarget{affil_58}{58}} Department of Physics, University of Warwick, Gibbet Hill Road, Coventry CV4 7AL, United Kingdom\\
\textsuperscript{\hypertarget{affil_59}{59}} Cavendish Laboratory, JJ Thomson Avenue, Cambridge CB3 0HE, UK\\
\textsuperscript{\hypertarget{affil_60}{60}} ESTEC, European Space Agency, 2201AZ, Noordwijk, NL\\
\textsuperscript{\hypertarget{affil_61}{61}} Center for Astronomy and Astrophysics, Technical University Berlin, Hardenberstrasse 36, 10623 Berlin, Germany\\
\textsuperscript{\hypertarget{affil_62}{62}} ELTE Eötvös Loránd University, Gothard Astrophysical Observatory, 9700 Szombathely, Szent Imre h. u. 112, Hungary\\
\textsuperscript{\hypertarget{affil_63}{63}} MTA-ELTE Exoplanet Research Group, 9700 Szombathely, Szent Imre h. u. 112, Hungary\\
\textsuperscript{\hypertarget{affil_64}{64}} Space sciences, Technologies and Astrophysics Research (STAR) Institute, Universit\'e de Li\`ege, 19C All\'ee du 6 Ao\^ut, B-4000 Li\`ege, Belgium\\
\textsuperscript{\hypertarget{affil_65}{65}} Institute of Astronomy, University of Cambridge, Madingley Road, Cambridge, CB3 0HA, United Kingdom\\
\textsuperscript{\hypertarget{affil_66}{66}} Department of Astrophysical Sciences, Princeton University, 4 Ivy Lane, Princeton, NJ 08544, USA\\
\textsuperscript{\hypertarget{affil_67}{67}} Department of Physics \& Astronomy, Swarthmore College, Swarthmore PA 19081, USA\\


==> oldauthors.tex <==

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%.    WARNING:  DO NOT EDIT YOUR AUTHOR INFO HERE.    %
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
% Author info is auto-generated from this google spreadsheet: https://docs.google.com/spreadsheets/d/1UoPGkxtxbHmJyDH8xKfOBbkoSoMXxiD9iDZ9ilVN0tE/edit?usp=sharing 
%
\author[H.~P.~Osborn et al.]{
\parbox{\textwidth}{
H.~P.~Osborn\textsuperscript{\hyperlink{affil_1}{1} , \hyperlink{affil_2}{2},,\orcidicon{0000-0002-4047-4724}}\thanks{E-mail:hugh.osborn@unibe.ch}, % hugh.osborn@unibe.ch First author
G.~Nowak\textsuperscript{{\hyperlink{affil_3}{3} , \hyperlink{affil_4}{4}}}, % gnowak@iac.es HARPS-N RV PI
G.~Hébrard\textsuperscript{{\hyperlink{affil_5}{5}}}, % hebrard@iap.fr Sophie RV PI
T.~Masseron\textsuperscript{{\hyperlink{affil_3}{3} , \hyperlink{affil_4}{4}}}, % thomas.masseron@iac.es HARPS-N RVs & stellar params
J.~Lillo~Box\textsuperscript{{\hyperlink{affil_6}{6},\orcidicon{0000-0003-3742-1987}}}, % jlillo@cab.inta-csic.es CAFE PI
E.~Pallé\textsuperscript{{\hyperlink{affil_3}{3} , \hyperlink{affil_7}{7},\orcidicon{0000-0003-0987-1593}}}, % epalle@iac.es HARPS-N RVs and Cheops GTO team
A.~Bekkelien\textsuperscript{{\hyperlink{affil_8}{8}}}, % Anja.Bekkelien@unige.ch Cheops Science Enabler
H.-G.~Florén\textsuperscript{{\hyperlink{affil_9}{9}}}, % floren@astro.su.se Cheops Science Enabler
P.~Guterman\textsuperscript{{\hyperlink{affil_10}{10}}}, % pascal.guterman@lam.fr Cheops Science Enabler
A.~E.~Simon\textsuperscript{{\hyperlink{affil_1}{1},\orcidicon{0000-0001-9773-2600}}}, % attila.simon@unibe.ch Cheops Science Enabler
V.~Adibekyan\textsuperscript{{\hyperlink{affil_11}{11},\orcidicon{0000-0002-0601-6199}}}, % Vardan.Adibekyan@astro.up.pt Stellar abundances and ages
A.~Bieryla\textsuperscript{{\hyperlink{affil_12}{12},\orcidicon{0000-0001-6637-5401}}}, % abieryla@cfa.harvard.edu TRES stellar parameters
A.~Brandeker\textsuperscript{{\hyperlink{affil_9}{9},\orcidicon{0000-0002-7201-7536}}}, % alexis@astro.su.se Cheops GTO team
D.~R.~Ciardi\textsuperscript{{\hyperlink{affil_13}{13},\orcidicon{0000-0002-5741-3047}}}, % ciardi@ipac.caltech.edu Palomar and Keck NIR AO data
A.~Collier~Cameron\textsuperscript{{\hyperlink{affil_14}{14},\orcidicon{0000-0002-8863-7828}}}, % acc4@st-andrews.ac.uk Cheops GTO team
K.~A.~Collins\textsuperscript{{\hyperlink{affil_12}{12},\orcidicon{0000-0001-6588-9574}}}, % karen.collins@cfa.harvard.edu SG1 coordination and data analysis
J.~A.~Egger\textsuperscript{{\hyperlink{affil_1}{1}}}, % jo-ann.egger@unibe.ch Interior structure modelling
D.~Gandolfi\textsuperscript{{\hyperlink{affil_15}{15},\orcidicon{0000-0001-8627-9628}}}, % davide.gandolfi@unito.it Advisor to Cheops duotransits team \& Explore Program manager
M.~J.~Hooton\textsuperscript{{\hyperlink{affil_16}{16} , \hyperlink{affil_1}{1},\orcidicon{0000-0003-0030-332X}}}, % matthew.hooton@unibe.ch Support with atmospheric potential
D.~W.~Latham\textsuperscript{{\hyperlink{affil_12}{12},\orcidicon{0000-0001-9911-7388}}}, % dlatham@cfa.harvard.edu TESS architects
M.~Lendl\textsuperscript{{\hyperlink{affil_17}{17},\orcidicon{0000-0001-9699-1459}}}, % monika.lendl@oeaw.ac.at Advisor to Cheops duotransits team
E.~Matthews\textsuperscript{{\hyperlink{affil_17}{17},\orcidicon{0000-0003-0593-1560}}}, % elisabeth.matthews@unige.ch Companion discussions
A.~Tuson\textsuperscript{{\hyperlink{affil_16}{16},\orcidicon{0000-0002-2830-9064}}}, % alt59@cam.ac.uk Key member of Cheops duotransits team
S.~Ulmer-Moll\textsuperscript{{\hyperlink{affil_17}{17},\orcidicon{0000-0003-2417-7006}}}, % solene.ulmer-moll@unige.ch Key member of Cheops duotransits team
A.~Vanderburg\textsuperscript{{\hyperlink{affil_2}{2}}}, % andrew.m.vanderburg@gmail.com Quaternion Detrending
T.~G.~Wilson\textsuperscript{{\hyperlink{affil_14}{14},\orcidicon{0000-0001-8749-1962}}}, % tgw1@st-andrews.ac.uk Stellar parameters
C.~Ziegler\textsuperscript{{\hyperlink{affil_18}{18}}}, % carlziegler@gmail.com LCO + SOAR
Y.~Alibert\textsuperscript{{\hyperlink{affil_1}{1},\orcidicon{0000-0002-4644-8818}}}, % yann.alibert@unibe.ch Cheops GTO team
R.~Alonso\textsuperscript{{\hyperlink{affil_3}{3} , \hyperlink{affil_4}{4},\orcidicon{0000-0001-8462-8126}}}, % ras@iac.es Cheops GTO team
G.~Anglada\textsuperscript{{\hyperlink{affil_19}{19} , \hyperlink{affil_20}{20}}}, % anglada@ice.csic.es Cheops GTO team
L.~Arnold\textsuperscript{{\hyperlink{affil_21}{21}}}, % Luc.Arnold@osupytheas.fr Sophie
J.~Asquier\textsuperscript{{\hyperlink{affil_22}{22}}}, % joel.asquier@esa.int Rando (MA) nomination
D.~Barrado~y~Navascues\textsuperscript{{\hyperlink{affil_23}{23}}}, % barrado@cab.inta-csic.es Cheops GTO team
W.~Baumjohann\textsuperscript{{\hyperlink{affil_24}{24},\orcidicon{0000-0001-6271-0110}}}, % baumjohann@oeaw.ac.at Cheops GTO team
T.~Beck\textsuperscript{{\hyperlink{affil_1}{1}}}, % thomas.beck@csh.unibe.ch Cheops GTO team
A.~A.~Belinski\textsuperscript{{\hyperlink{affil_25}{25},\orcidicon{0000-0003-3469-0989}}}, % aleks.sai@gmail.com SAI-2.5m speckle data
W.~Benz\textsuperscript{{\hyperlink{affil_1}{1} , \hyperlink{affil_26}{26}}}, % willy.benz@unibe.ch Cheops GTO team
A.~Bieryla\textsuperscript{{\hyperlink{affil_12}{12}}}, % abieryla@cfa.harvard.edu TRES spectra/stellar parameters
F.~Biondi\textsuperscript{{\hyperlink{affil_27}{27} , \hyperlink{affil_28}{28},\orcidicon{0000-0002-1337-3653}}}, % biondi@mpe.mpg.de Magrin (MA) nomination
I.~Boisse\textsuperscript{{\hyperlink{affil_29}{29}}}, % isabelle.boisse@lam.fr Sophie
X.~Bonfils\textsuperscript{{\hyperlink{affil_30}{30}}}, % xavier.bonfils@obs.ujf-grenoble.fr Cheops GTO team
C.~Broeg\textsuperscript{{\hyperlink{affil_1}{1} , \hyperlink{affil_26}{26},\orcidicon{0000-0001-5132-2614}}}, % christopher.broeg@unibe.ch Cheops GTO team
L.~A.~Buchhave\textsuperscript{{\hyperlink{affil_31}{31},\orcidicon{0000-0003-1605-5666}}}, % buchhave@space.dtu.dk FIES spectra
T.~Bárczy\textsuperscript{{\hyperlink{affil_32}{32}}}, % tamas.barczy@admatis.com Cheops GTO team
S.~C.~C.~Barros\textsuperscript{{\hyperlink{affil_33}{33} , \hyperlink{affil_34}{34},\orcidicon{0000-0003-2434-3625}}}, % susana.barros@astro.up.pt Cheops GTO team
J.~Cabrera\textsuperscript{{\hyperlink{affil_35}{35},\orcidicon{0000-0001-6653-5487}}}, % juan.cabrera@dlr.de Cheops GTO team
C.~Cardona~Guillen\textsuperscript{{\hyperlink{affil_3}{3} , \hyperlink{affil_7}{7}}}, % carlos.cardona@iac.es HARPS-N observer
I.~Carleo\textsuperscript{{\hyperlink{affil_3}{3} , \hyperlink{affil_7}{7}}}, % icarleo@iac.es HARPS-N observer
A.~Castro-González\textsuperscript{{\hyperlink{affil_6}{6},\orcidicon{0000-0001-7439-3618}}}, % acastro@cab.inta-csic.es CAFE
S.~Charnoz\textsuperscript{{\hyperlink{affil_36}{36}}}, % charnoz@ipgp.fr Cheops GTO team
J.~Christiansen\textsuperscript{{\hyperlink{affil_13}{13}}}, % christia@ipac.caltech.edu TESS/TSO nomination
P.~Cortes\textsuperscript{{\hyperlink{affil_29}{29}}}, % pia.cortes@lam.fr Sophie
S.~Csizmadia\textsuperscript{{\hyperlink{affil_35}{35}}}, % szilard.csizmadia@dlr.de Cheops GTO team
S.~Dalal\textsuperscript{{\hyperlink{affil_5}{5}}}, % shweta.dalal@iap.fr Sophie
M.~B.~Davies\textsuperscript{{\hyperlink{affil_37}{37},\orcidicon{0000-0001-6080-1190}}}, % melvyn_b.davies@math.lu.se Cheops GTO team
M.~Deleuil\textsuperscript{{\hyperlink{affil_38}{38}}}, % magali.deleuil@lam.fr Cheops GTO team
X.~Delfosse\textsuperscript{{\hyperlink{affil_39}{39}}}, % xavier.delfosse@univ-grenoble-alpes.fr Sophie
L.~Delrez\textsuperscript{{\hyperlink{affil_40}{40} , \hyperlink{affil_41}{41}}}, % ldelrez@uliege.be Cheops GTO team
B.-O.~Demory\textsuperscript{{\hyperlink{affil_42}{42}}}, % brice.demory@csh.unibe.ch Cheops GTO team
D.~Ehrenreich\textsuperscript{{\hyperlink{affil_17}{17}}}, % david.ehrenreich@unige.ch Cheops GTO team
A.~Erikson\textsuperscript{{\hyperlink{affil_35}{35}}}, % Anders.Erikson@dlr.de Cheops GTO team
R.~B.~Fernandes\textsuperscript{{\hyperlink{affil_43}{43},\orcidicon{0000-0002-3853-7327}}}, % rachelfernandes@email.arizona.edu Palomar NIR AO data
A.~Fortier\textsuperscript{{\hyperlink{affil_1}{1} , \hyperlink{affil_26}{26},\orcidicon{0000-0001-8450-3374}}}, % andrea.fortier@unibe.ch Cheops GTO team
T.~Forveille\textsuperscript{{\hyperlink{affil_39}{39}}}, % thierry.forveille@univ-grenoble-alpes.fr Sophie
L.~Fossati\textsuperscript{{\hyperlink{affil_24}{24}}}, % Luca.Fossati@oeaw.ac.at Cheops GTO team
M.~Fridlund\textsuperscript{{\hyperlink{affil_44}{44} , \hyperlink{affil_45}{45}}}, % fridlund@strw.leidenuniv.nl Cheops GTO team
E.~Furlan\textsuperscript{{\hyperlink{affil_13}{13}}}, % furlan@ipac.caltech.edu Gemini NIR AO data
M.~Gillon\textsuperscript{{\hyperlink{affil_40}{40}}}, % michael.gillon@ulg.ac.be Cheops GTO team
R.~F.~Goeke\textsuperscript{{\hyperlink{affil_2}{2}}}, % goeke@space.mit.edu TESS/POC nomination
M.~V.~Goliguzova\textsuperscript{{\hyperlink{affil_25}{25},\orcidicon{0000-0003-2228-7914}}}, % margo1000i1@mail.ru SAI-2.5m speckle data
E.~J.~Gonzales\textsuperscript{{\hyperlink{affil_46}{46},\orcidicon{0000-0002-9329-2190}}}, % erjagonz@ucsc.edu Keck NIR AO data
M.~Güdel\textsuperscript{{\hyperlink{affil_47}{47}}}, % manuel.guedel@univie.ac.at Cheops GTO team
N.~Heidari\textsuperscript{{\hyperlink{affil_29}{29}}}, % neda.heidari@lam.fr Sophie
S.~Howell\textsuperscript{{\hyperlink{affil_48}{48}}}, % steve.b.howell@nasa.gov Gemini
S.~Hoyer\textsuperscript{{\hyperlink{affil_38}{38}}}, % sergio.hoyer@lam.fr Cheops GTO team
J.~Immanuel~Frey\textsuperscript{{\hyperlink{affil_42}{42}}}, % jonas.frey@unibe.ch Beck (MA) nomination
K.~G.~Isaak\textsuperscript{{\hyperlink{affil_49}{49}}}, % kisaak@cosmos.esa.int Cheops/ESAPS author
J.~M.~Jenkins\textsuperscript{{\hyperlink{affil_48}{48},\orcidicon{0000-0002-4715-9460}}}, % jon.jenkins@nasa.gov TESS architects
F.~Kiefer\textsuperscript{{\hyperlink{affil_5}{5}}}, % kiefer@iap.fr Sophie
L.~Kiss\textsuperscript{{\hyperlink{affil_50}{50} , \hyperlink{affil_51}{51}}}, % kiss@konkoly.hu Cheops GTO team
J.~Korth\textsuperscript{{\hyperlink{affil_52}{52} , \hyperlink{affil_53}{53}}}, % judithkorth@googlemail.com HARPS-N observer
P.~F.~L.~Maxted\textsuperscript{{\hyperlink{affil_54}{54}}}, % p.maxted@keele.ac.uk Cheops GTO team
J.~Laskar\textsuperscript{{\hyperlink{affil_55}{55}}}, % laskar@imcce.fr Cheops GTO team
A.~Lecavelier~des~Etangs\textsuperscript{{\hyperlink{affil_56}{56}}}, % lecaveli@iap.fr Cheops GTO team
C.~Lovis\textsuperscript{{\hyperlink{affil_17}{17}}}, % christophe.lovis@unige.ch Cheops GTO team
M.~B.~Lund\textsuperscript{{\hyperlink{affil_13}{13},\orcidicon{0000-0002-4236-9020}}}, % mlund@ipac.caltech.edu Palomar NIR AO data
R.~Luque\textsuperscript{{\hyperlink{affil_57}{57}}}, % rluque@uchicago.edu HARPS-N observer
D.~Magrin\textsuperscript{{\hyperlink{affil_58}{58}}}, % demetrio.magrin@inaf.it Cheops GTO team
J.~Manuel~Almenara\textsuperscript{{\hyperlink{affil_39}{39}}}, % jose-manuel.almenara-villa@univ-grenoble-alpes.fr Sophie
E.~Martioli\textsuperscript{{\hyperlink{affil_5}{5} , \hyperlink{affil_59}{59}}}, % martioli@iap.fr Sophie
M.~Mecina\textsuperscript{{\hyperlink{affil_47}{47}}}, % marko.mecina@univie.ac.at Ottensamer (Cheops MA) nomination
J.~V.~Medina\textsuperscript{{\hyperlink{affil_60}{60}}}, % jmedina@stsci.edu TESS/POC nomination
D.~Moldovan\textsuperscript{{\hyperlink{affil_61}{61}}}, % mdan@google.com TESS/POC nomination
M.~Morales-Calder\'on\textsuperscript{{\hyperlink{affil_6}{6}}}, % mariamc@cab.inta-csic.es CAFE
G.~Morello\textsuperscript{{\hyperlink{affil_3}{3} , \hyperlink{affil_7}{7}}}, % giuseppe.morello@iac.es HARPS-N observer
C.~Moutou\textsuperscript{{\hyperlink{affil_62}{62}}}, % claire.moutou@irap.omp.eu Sophie
F.~Murgas\textsuperscript{{\hyperlink{affil_3}{3} , \hyperlink{affil_7}{7}}}, % fmurgas@iac.es HARPS-N observer
E.~L.~N.~Jensen\textsuperscript{{\hyperlink{affil_63}{63},\orcidicon{0000-0002-4625-7333}}}, % ejensen1@swarthmore.edu LCO observations
V.~Nascimbeni\textsuperscript{{\hyperlink{affil_58}{58},\orcidicon{0000-0001-9770-1214}}}, % valerio.nascimbeni@inaf.it Cheops GTO team
G.~Olofsson\textsuperscript{{\hyperlink{affil_9}{9}}}, % olofsson@astro.su.se Cheops GTO team
R.~Ottensamer\textsuperscript{{\hyperlink{affil_47}{47}}}, % roland.ottensamer@univie.ac.at Cheops GTO team
I.~Pagano\textsuperscript{{\hyperlink{affil_64}{64}}}, % isabella.pagano@inaf.it Cheops GTO team
G.~Peter\textsuperscript{{\hyperlink{affil_35}{35}}}, % gisbert.peter@dlr.de Cheops GTO team
G.~Piotto\textsuperscript{{\hyperlink{affil_65}{65} , \hyperlink{affil_58}{58}}}, % giampaolo.piotto@unipd.it Cheops GTO team
D.~Pollacco\textsuperscript{{\hyperlink{affil_66}{66}}}, % d.pollacco@warwick.ac.uk Cheops GTO team
D.~Queloz\textsuperscript{{\hyperlink{affil_17}{17} , \hyperlink{affil_67}{67}}}, % didier.queloz@unige.ch Cheops GTO team
R.~Ragazzoni\textsuperscript{{\hyperlink{affil_58}{58} , \hyperlink{affil_65}{65}}}, % roberto.ragazzoni@inaf.it Cheops GTO team
N.~Rando\textsuperscript{{\hyperlink{affil_22}{22}}}, % nicola.rando@esa.int Cheops GTO team
H.~Rauer\textsuperscript{{\hyperlink{affil_35}{35} , \hyperlink{affil_68}{68}}}, % Heike.Rauer@dlr.de Cheops GTO team
I.~Ribas\textsuperscript{{\hyperlink{affil_19}{19} , \hyperlink{affil_20}{20}}}, % iribas@ice.cat Cheops GTO team
G.~Ricker\textsuperscript{{\hyperlink{affil_2}{2},\orcidicon{0000-0003-2058-6662}}}, % grr@space.mit.edu TESS architects
O.~D.~S.~Demangeon\textsuperscript{{\hyperlink{affil_33}{33} , \hyperlink{affil_34}{34},\orcidicon{0000-0001-7918-0355}}}, % olivier.demangeon@astro.up.pt Cheops GTO team
A.~M.~S.~Smith\textsuperscript{{\hyperlink{affil_35}{35},\orcidicon{0000-0002-2386-4341}}}, % alexis.smith@dlr.de Cheops GTO team
N.~Santos\textsuperscript{{\hyperlink{affil_33}{33} , \hyperlink{affil_34}{34}}}, % nuno.santos@astro.up.pt Cheops GTO team
G.~Scandariato\textsuperscript{{\hyperlink{affil_64}{64},\orcidicon{0000-0003-2029-0626}}}, % gaetano.scandariato@inaf.it Cheops GTO team
S.~Seager\textsuperscript{{\hyperlink{affil_2}{2},\orcidicon{0000-0002-6892-6948}}}, % seager@mit.edu TESS architects
S.~G.~Sousa\textsuperscript{{\hyperlink{affil_33}{33},\orcidicon{0000-0001-9047-2965}}}, % sergio.sousa@astro.up.pt Stellar parameters
M.~Steller\textsuperscript{{\hyperlink{affil_24}{24}}}, % Manfred.Steller@oeaw.ac.at Cheops GTO team
G.~M.~Szabó\textsuperscript{{\hyperlink{affil_69}{69} , \hyperlink{affil_70}{70}}}, % szgy@konkoly.hu; szgy@gothard.hu Cheops GTO team
D.~Ségransan\textsuperscript{{\hyperlink{affil_17}{17}}}, % damien.segransan@unige.ch Cheops GTO team
N.~Thomas\textsuperscript{{\hyperlink{affil_1}{1}}}, % nicolas.thomas@unibe.ch Cheops GTO team
S.~Udry\textsuperscript{{\hyperlink{affil_17}{17},\orcidicon{0000-0001-7576-6236}}}, % stephane.udry@unige.ch Cheops GTO team
B.~Ulmer\textsuperscript{{\hyperlink{affil_71}{71}}}, % bernd.ulmer@dlr.de Gisbert (MA) nomination
V.~Van~Grootel\textsuperscript{{\hyperlink{affil_41}{41},\orcidicon{0000-0003-2144-4316}}}, % valerie.vangrootel@uliege.be Stellar parameters
R.~Vanderspek\textsuperscript{{\hyperlink{affil_2}{2},\orcidicon{0000-0001-6763-6562}}}, % roland@space.mit.edu TESS architects
N.~Walton\textsuperscript{{\hyperlink{affil_72}{72}}}, % naw@ast.cam.ac.uk Cheops GTO team
J.~N.~Winn\textsuperscript{{\hyperlink{affil_73}{73},\orcidicon{0000-0002-4265-047X}}}% jnwinn@princeton.edu TESS architects
}
\\
% List of institutions
Affiliations are listed at the end of the paper in Appendix \ref{sec:affiliations}.
}

==> oldpaper <==

\newcommand{\gcm}{g\,cm$^{-3}$}	% g per cm-cubed
\newcommand\todo[1]{\textcolor{red}{\textbf{#1}}}
\newcommand{\kepler}{{\it Kepler}}
\newcommand{\corot}{{\it CoRoT}}
\newcommand{\tess}{{\it TESS}}
\newcommand{\plato}{{\it PLATO}}
\newcommand{\gaia}{{\it Gaia}}
\newcommand{\JWST}{{\it JWST}}
\newcommand{\ktwo}{{\it K2}}
\newcommand{\cheops}{{\it CHEOPS}}

\newcommand{\kms}{km\,s$^{-1}$}
\newcommand{\ms}{m\,s$^{-1}$}
\newcommand{\mss}{\mbox{m\,s$^{-2}$}}
\newcommand{\masy}{mas\,yr$^{-1}$}
\newcommand{\mpl}{\mbox{$M_{p}$}}
\newcommand{\rpl}{\mbox{$R_{p}$}}
\newcommand{\mstar}{\mbox{$M_{\star}$}}
\newcommand{\rstar}{\mbox{$R_{\star}$}}
\newcommand{\mjup}{\mbox{$M_{\rm Jup}$}}
\newcommand{\rjup}{\mbox{$R_{\rm Jup}$}}
\newcommand{\msun}{\mbox{$M_{\odot}$}}
\newcommand{\rsun}{\mbox{$R_{\odot}$}}
\newcommand{\rearth}{R$_{\oplus}$}
\newcommand{\mearth}{M$_{\oplus}$}
\newcommand{\gccc}{g\,cm$^{-3}$}
\newcommand{\ergscm}{erg\,s$^{-1}$cm$^{-2}$}
\newcommand{\vsini}{$v\sin{i}$}
\newcommand{\teff}{$T_{\rm eff}$}
\newcommand{\feh}{\mbox{$\rm [Fe/H]$}}
\newcommand{\ymg}{\mbox{$\rm [Y/Mg]$}}
\newcommand{\logg}{$\log g$}
\newcommand{\rprs}{\mbox{R$_{p}/$R$_{s}$}}
\newcommand{\vdag}{(v)^\dagger}

\newcommand{\TTstar}{TOI-1471}
\newcommand{\Tstarage}{99\,$\pm$\,0.5 Gyr}
\newcommand{\monotools}{\texttt{MonoTools}}
\newcommand{\celerite}{\textit{celerite}}
\newcommand{\refcomb}{}
\newcommand{\refcom}{}

\include{macro}

\newcommand{\pminc}{$17.2$}
\newcommand{\pmaxc}{$189.1$}
\newcommand{\pmind}{$25.1 $}
\newcommand{\pmaxd}{$175.6 $}
\newcommand{\bcloglikratio}{$101.7$}

\title{<- CLICK ON \_PAPER.tex}
\author{Hugh Osborn}
\date{May 2022}

\section{CLICK ON \_PAPER.tex}

\textbf{CLICK ON \_PAPER.tex}

Transiting planets are key to the near future of exoplanet characterisation, especially with the success of JWST.
Planets at short orbital distances are now known in abundance around bright stars thanks to both ground-based transit surveys (for Giant planets) and \tess{}.

In the Neptune-like planets will provide a key intermediate between gas giants

Initially detected at 11.767d

\section{Data}




\section{Analysis}


\begin{table}
\caption{Derived stellar parameters.}  % title of Table
\label{table:star_params}      % is used to refer this table in the text
\centering                          % used for centering table
\begin{tabular}{l c c }        % centred columns (4 columns)
\hline\hline                 % inserts double horizontal lines
Parameter & Value & source \\
\hline                        % inserts single horizontal line
Name & HD 12572 \\
TIC & \TICstar{}$^{\dagger}$ \\
\textit{BD} designation & BD+40 2790 \\
\gaia{} DR2 ID & 1490845442647992960 $^{\star}$ \\
RA [$^\circ$, J2015.5] & 217.391994602 $^{\star}$ \\
Dec [$^\circ$, J2015.5] & 39.790398204 $^{\star}$ \\
\tess{} mag & $8.3745 \pm 0.006$\,$^{\dagger}$\\
\textit{G} mag & $8.92\pm0.000477$\,$^{\star}$ \\
\textit{K} mag & $7.115\pm0.017$\,$^{\ddagger}$\\
\teff{} [K] & $5200\pm70$\,$^{\beta}$\\
$R_s$ [$R_\odot$] & $0.77\pm0.006$\,$^{\beta}$\\
$M_s$ [$M_\odot$] & $0.824_{-0.037}^{+0.035}$\,$^{\beta}$\\
\logg{} [cgs] & $4.45\pm0.12$\,$^{\beta}$\\
$[{\rm Fe}/{\rm H}]$ & $-0.09\pm0.04$\,$^{\beta}$\\
$\log{\rm R'HK}$ [dex] & $-4.373\pm0.02$\,$^{\beta}$ \\
Gyrochron. Age [Gyr] & $0.204\pm0.050$\,$^{\alpha}$\\
$\log{\rm R'HK}$ Age [Gyr] & $0.42\pm0.13$\,$^{\beta}$\\
Adopted Age [Gyr] & $0.34\pm 0.08$\,$^{\beta}$\\
\hline                                   %inserts single line
\end{tabular}
\begin{tablenotes}
\small
\item Notation refers to the following sources: $^{\star}$ Gaia EDR3 \citep{2021A&A...649A...1G}; $^{\dagger}$ TESS Input Catalog  \citep{2018AJ....156..102S}; $^{\ddagger}$ 2MASS  \citep{2003tmc..book.....C}; $^{\alpha}$ analysis by H21; $^{\beta}$ Our own analysis as described in Section \ref{sect:starpars}.
\end{tablenotes}
\end{table}

\section{Discussion}
\subsection{RV drift}
We measure a sizable RV drift of $-19.2\rm{m.s}^{-1}$ per year.
Comparisons of combined models with linear and quadratic RV trends also shows that the RV drift prefers a model with curvature ($-0.7\pm0.05m.s{^-s}.yr^{-1}.yr^{-1}$).
Curvature over a 10-year baseline suggests a likely orbital period on the order of 100s of years, and the drift amplitude suggests a companion within the brown dwarf regime.
This implies that there any added dilution required is extremely minimal, as the luminosities of even low-mass M-dwarfs are minimal in the TESS and Cheops bandpasses.
The current RV curvature also implies that the companion may be approaching conjunction, which would explain why high-resolution imaging does not detect any such object.

One complication comes from the fact that the Hipparchos-Gaia catalogue of accelerations finds only a very minimal deviation from a linear ephemeris (2.647 chi-square difference) and the Gaia EDR3 astrometric\_chi\_sq value(ruwe) of 1.03 very likely suggests single star.

%- implies either low-mass or long period (such that deviations over 25+ year baseline would not produce measured accelerations).
%However, we rule out nearby-companions to only 0.5" ($\sim32$AU), below which stellar companions should produce measurable acceleration (or RV non-linearity) over a 10-year baseline.


One interesting 
%TOI-402, which shows a similar though less-pronounced RV drift (though has a measured companion at 0.6"), has a chi-squared value of 481 against a linear model in the HGCA.


Two possibilities:
1) Velocity vector unchanged, i.e. change in motion between Gaia \& Hipparchos ephemerides minimal due to long-period massive companion
2) Short variation timescale at low amplitude, i.e. any change in motion between Gaia and Hipparchos ephemerides is below 

For 1) timescale is 25yrs. For an orbit of >150yrs and a position far from quadrature, this could be possible.

EDR3 detection (Gaia DR2 94469008266498944) only 2.2 arcsecs away at G=16.38. No parallax or astrometry. DeltaMag=7.35, so contributes 1.18ppt of light. Therefore too faint to cause observed transits (1.5-2ppt).
DR3 shows 6.14-sigma excess noise, however this corresponds to only 80microarseconds = 1.2 solar radii; consistent with a giant planet.

\subsection{Search for TTVs}
None detected at <5min

\section{Conclusion}

\maketitle

\section{Introduction}

\section{appendix}

\begin{table*}
\tiny
\caption{Model parameters, priors and posteriors for the Combined model}             % title of Table
\label{table:appendix_P35_model2}      % is used to refer this table in the text
\centering                          % used for centering table
\begin{tabular}{l c c}        % centred columns (4 columns)
\hline\hline                 % inserts double horizontal lines
Parameter & Prior & Posterior \\
\hline                        % inserts single horizontal line
\input{priorpost.tex}
\hline                                   %inserts single line
\end{tabular}
\begin{caption}
      \tiny
      \item $\mathcal{N}$ details a normally distributed prior with mean, $\mu$ and standard deviation, $\sigma$ values. $\mathcal{U}$ details a uniform distribution with lower, $a$, and upper, $b$, limits. $\mathcal{N}_\mathcal{U}$ details a truncated normal distribution with $\mu$,$\sigma$, $a$ \& $b$ values.$\ddagger{}$ represents the uniform prior as presented by \citet{2018RNAAS...2..209E} and implemented by \texttt{exoplanet}.
    \end{caption}
\end{table*}


==> priorpost.tex <==
Stellar temperature, \teff{}  [K]  & $\mathcal{N}(\mu=5610,\sigma=30) $ &  $ 5611.0 \pm 31.0 $  \\
Stellar radius, $R_s$ [$R_\oplus$] & $\mathcal{N}(\mu=0.9662,\sigma=0.005) $ &  $ 0.9662 \pm 0.0048 $  \\
log stellar surface gravity, \logg{}  [cgs] & $\mathcal{N}(\mu=4.47,\sigma=0.1) $ &  $ 4.45^{+0.016}_{-0.036} $  \\
Log RV semi-amplitude, $\log{K}$ & $\mathcal{N}(\mu=0.693147,\sigma=10)$ &  $ 1.34^{+0.12}_{-0.15} $  \\
Log RV semi-amplitude, $\log{K}$ & $\mathcal{N}(\mu=0.693147,\sigma=10)$ &  $ -0.9^{+1.0}_{-8.7} $  \\
Quadratic LD, $u_{{\rm TESS},0} $  & $\mathcal{N}_{\mathcal{U}}(a=0.0,b=1.0,\mu=0.3306,\sigma=0.0500)$ &  $ 0.303^{+0.061}_{-0.068} $  \\
Quadratic LD, $u_{{\rm TESS},1} $  & $\mathcal{N}_{\mathcal{U}}(a=0.0,b=1.0,\mu=0.2602,\sigma=0.0500)$ &  $ 0.22 \pm 0.087 $  \\
Quadratic LD, $u_{{\rm Cheops},0} $  & $\mathcal{N}_{\mathcal{U}}(a=0.0,b=1.0,\mu=0.4494,\sigma=0.0500)$ &  $ 0.498 \pm 0.064 $  \\
Quadratic LD, $u_{{\rm Cheops},1} $  & $\mathcal{N}_{\mathcal{U}}(a=0.0,b=1.0,\mu=0.2292,\sigma=0.0500)$ &  $ 0.205 \pm 0.081 $  \\
RV mean, $\mu_{\rm Sophie}$ & $\mathcal{N}(\mu=-16077.1,\sigma=271.527)$ &  $ -16082.61 \pm 0.58 $  \\
RV mean, $\mu_{\rm HARPS-N}$ & $\mathcal{N}(\mu=-2.8479,\sigma=112.492)$ &  $ -11.38 \pm 0.35 $  \\
quadratic RV trend term quadratic & $\mathcal{N}(\mu=0,\sigma=0.005)$ &  $ -5.22e-06 \pm 3.8e-07 $  \\
linear RV trend term linear & $\mathcal{N}(\mu=0,\sigma=0.05)$ &  $ -0.067 \pm 0.001 $  \\
Log photometric scatter, $\log{\sigma_{{\rm TESS},s}/(\rm{ppt})}$  & $\mathcal{N}(\mu=0.1484,\sigma=3) $ &  $ -0.579 \pm 0.012 $  \\
Trend with normalised sine of roll angle, $df/d({\sin{\Phi}})_N$   & $\mathcal{N}(\mu=0,\sigma=1) $ &  $ -0.013^{+0.036}_{-0.034} $  \\
Trend with normalised cosine of roll angle, $df/d({\cos{\Phi}})_N$   & $\mathcal{N}(\mu=0,\sigma=1) $ &  $ 0.064 \pm 0.026 $  \\
Trend with normalised background flux, $df/d({\cos{\Phi}})_N$   & $\mathcal{N}(\mu=0,\sigma=1) $ &  $ 0.71 \pm 0.92 $  \\
Mean flux, $\mu_{{\rm Cheops}}$ [ppt]  & $\mathcal{N}(\mu=0,\sigma=0.3127) $ &  $ 0.423 \pm 0.027 $  \\
Log photometric scatter, $\log{\sigma_{{\rm Cheops},s}/(\rm{ppt})}$  & $\mathcal{N}(\mu=-1.469,\sigma=3) $ &  $ -2.11^{+0.15}_{-0.19} $  \\


==> table-TOI-1471-tng_harpn-0013-srv-drs-complete_output.tex <==
\begin{table*}
%\begin{sidewaystable}
%\begin{footnotesize}
%\begin{scriptsize}
%\begin{ssmall}
\begin{tiny}
\begin{center}
\caption{Radial velocities and spectral activity indicators measured from TNG/HARPS-N spectra with SERVAL and DRS.
\label{table-TOI-1471-tng_harpn-0013-srv-drs-complete_output}}
\begin{tabular}{rrrrrrrrrrrrrrrrrrrrr}
\hline
\hline
%\noalign{\smallskip}
\multicolumn{1}{c}{BJD$_\mathrm{TBD}$} &
\multicolumn{2}{c}{RV} &
\multicolumn{2}{c}{BIS} &
\multicolumn{1}{c}{CCF\_FWHM} &
\multicolumn{1}{c}{CCF\_CTR} &
\multicolumn{2}{c}{$\mathrm{\log{R^{`}_{HK}}}$} &
\multicolumn{2}{c}{CRX} &
\multicolumn{2}{c}{dlW} &
\multicolumn{2}{c}{$\mathrm{H_{\alpha}}$} &
\multicolumn{2}{c}{$\mathrm{NaD_{1}}$} &
\multicolumn{2}{c}{$\mathrm{NaD_{2}}$} &
\multicolumn{1}{c}{SNR} &
\multicolumn{1}{c}{$\mathrm{T_{exp}}$}\\ 
\multicolumn{1}{c}{-2457000} &
\multicolumn{2}{c}{($\mathrm{m\,s^{-1}}$)} &
\multicolumn{2}{c}{($\mathrm{m\,s^{-1}}$)} &
\multicolumn{1}{c}{($\mathrm{km\,s^{-1}}$)} &
\multicolumn{1}{c}{(\%)} &
\multicolumn{2}{c}{---} &
\multicolumn{2}{c}{($\mathrm{m\,s^{-1}\,Np^{-1}}$)} &
\multicolumn{2}{c}{($\mathrm{m^2\,s^{-2}}$)} &
\multicolumn{2}{c}{---} &
\multicolumn{2}{c}{---} &
\multicolumn{2}{c}{---} &
\multicolumn{1}{c}{(@550nm)} &
\multicolumn{1}{c}{(s)}\\ 
\multicolumn{1}{c}{Val.} &
\multicolumn{1}{c}{Val.} &
\multicolumn{1}{c}{$\sigma$} &
\multicolumn{1}{c}{Val.} &
\multicolumn{1}{c}{$\sigma$} &
\multicolumn{1}{c}{Val.} &
\multicolumn{1}{c}{Val.} &
\multicolumn{1}{c}{Val.} &
\multicolumn{1}{c}{$\sigma$} &
\multicolumn{1}{c}{Val.} &
\multicolumn{1}{c}{$\sigma$} &
\multicolumn{1}{c}{Val.} &
\multicolumn{1}{c}{$\sigma$} &
\multicolumn{1}{c}{Val.} &
\multicolumn{1}{c}{$\sigma$} &
\multicolumn{1}{c}{Val.} &
\multicolumn{1}{c}{$\sigma$} &
\multicolumn{1}{c}{Val.} &
\multicolumn{1}{c}{$\sigma$} &
\multicolumn{1}{c}{Val.} &
\multicolumn{1}{c}{Val.}\\ 
%\noalign{\smallskip}
\hline
%\noalign{\smallskip}
    1869.319080 &           7.274 &           1.594 &         -27.281 &           2.682 &           6.780 &          47.865 &         -4.9633 &          0.0205 &          29.887 &          11.583 &         -37.889 &           3.935 &          0.4301 &          0.0016 &          0.3149 &          0.0019 &          0.4175 &          0.0024 &            47.9 &           281.1\\
    1869.335750 &           5.772 &           0.806 &         -25.601 &           1.109 &           6.779 &          47.942 &         -4.9847 &          0.0060 &           2.627 &           6.214 &         -41.656 &           2.271 &          0.4286 &          0.0007 &          0.3137 &          0.0009 &          0.4150 &          0.0011 &           105.3 &          1500.0\\
    1895.396750 &          -2.848 &           1.292 &         -27.726 &           1.941 &           6.781 &          48.022 &         -5.0056 &          0.0160 &           5.731 &           9.725 &         -56.570 &           3.409 &          0.4321 &          0.0011 &          0.3174 &          0.0014 &          0.4210 &          0.0018 &            63.7 &          1500.0\\
    1896.386300 &          -2.531 &           0.880 &         -24.883 &           1.484 &           6.787 &          47.982 &         -4.9759 &          0.0097 &         -11.668 &           6.324 &         -47.814 &           2.940 &          0.4307 &          0.0008 &          0.3140 &          0.0011 &          0.4141 &          0.0013 &            81.1 &          1500.0\\
    1897.382590 &          -2.646 &           0.746 &         -22.277 &           1.326 &           6.777 &          47.980 &         -4.9577 &          0.0078 &          -0.995 &           5.610 &         -46.034 &           2.398 &          0.4292 &          0.0008 &          0.3125 &          0.0010 &          0.4167 &          0.0012 &            90.5 &          1500.0\\
    1898.387220 &          -0.632 &           0.764 &         -25.694 &           1.108 &           6.783 &          47.944 &         -4.9640 &          0.0059 &          -8.666 &           5.588 &         -43.342 &           2.247 &          0.4301 &          0.0006 &          0.3144 &          0.0008 &          0.4251 &          0.0010 &           107.3 &          1500.0\\
    1905.364120 &           2.234 &           1.464 &         -28.000 &           2.216 &           6.778 &          47.951 &         -4.9860 &          0.0191 &          13.930 &          11.157 &         -41.969 &           3.183 &          0.4297 &          0.0013 &          0.3223 &          0.0016 &          0.4286 &          0.0020 &            57.5 &          1723.9\\
    2548.360870 &         -40.913 &           1.851 &         -33.469 &           2.750 &           6.768 &          48.124 &         -5.0687 &          0.0392 &           5.014 &          15.357 &         -64.478 &           4.110 &          0.4361 &          0.0017 &          0.3313 &          0.0019 &          0.4366 &          0.0024 &            51.1 &          2400.0\\
    2574.431260 &         -46.649 &           3.096 &         -35.382 &           6.024 &           6.777 &          47.795 &         -4.8758 &          0.0726 &          63.574 &          26.024 &         -31.740 &           6.085 &          0.4392 &          0.0039 &          0.3541 &          0.0040 &          0.4744 &          0.0052 &            28.4 &           680.8\\
    2574.451860 &         -42.020 &           1.468 &         -32.075 &           2.098 &           6.768 &          47.980 &         -4.9197 &          0.0205 &         -11.941 &          12.857 &         -42.810 &           3.729 &          0.4376 &          0.0014 &          0.3330 &          0.0015 &          0.4572 &          0.0020 &            66.6 &          1800.0\\
    2594.453560 &         -44.065 &           1.613 &         -29.413 &           2.151 &           6.769 &          47.996 &         -4.9653 &          0.0215 &          -0.885 &          13.713 &         -51.564 &           2.602 &          0.4307 &          0.0014 &          0.3138 &          0.0015 &          0.4264 &          0.0019 &            63.3 &          1200.0\\
    2609.385030 &         -45.321 &           2.642 &         -29.236 &           3.610 &           6.776 &          48.181 &         -5.0135 &          0.0504 &           3.432 &          21.351 &         -66.118 &           5.144 &          0.4318 &          0.0019 &          0.3158 &          0.0023 &          0.4306 &          0.0030 &            40.9 &           600.0\\
    2610.395010 &         -43.474 &           1.115 &         -33.068 &           1.609 &           6.772 &          48.079 &         -4.9536 &          0.0119 &          -1.577 &           9.376 &         -56.704 &           2.282 &          0.4293 &          0.0010 &          0.3151 &          0.0011 &          0.4275 &          0.0014 &            81.8 &           600.0\\
%\noalign{\smallskip}
\hline
\end{tabular}
\end{center}
%\end{footnotesize}
%\end{scriptsize}
%\end{ssmall}
\end{tiny}
%\end{sidewaystable}
\end{table*}

